NOD-TAMP: Generalizable Long-Horizon Planning with Neural Object Descriptors

Solving complex manipulation tasks in household and factory settings remains challenging due to long-horizon reasoning, fine-grained interactions, and broad object and scene diversity. Learning skills from demonstrations can be an effective strategy, but such methods often have limited generalizability beyond training data and struggle to solve long-horizon tasks. To overcome this, we propose to synergistically combine two paradigms: Neural Object Descriptors (NODs) that produce generalizable object-centric features and Task and Motion Planning (TAMP) frameworks that chain short-horizon skills to solve multi-step tasks. We introduce NOD-TAMP, a TAMP-based framework that extracts short manipulation trajectories from a handful of human demonstrations, adapts these trajectories using NOD features, and composes them to solve broad long-horizon, contact-rich tasks. NOD-TAMP solves existing manipulation benchmarks with a handful of demonstrations and significantly outperforms prior NOD-based approaches on new tabletop manipulation tasks that require diverse generalization. Finally, we deploy NOD-TAMP on a number of real-world tasks, including tool-use and high-precision insertion. For more details, please visit https://nodtamp.github.io/.

==> text/Algm1.tex <==

\begin{algorithm}[!ht]
  \begin{small} % footnotesize
  \caption{Trajectory adaptation}
  \label{alg:adaptation}
  \begin{algorithmic}[1] % The number tells where the line numbering should start
    % \Declare Segmented point clouds $\overline{{\cal P}}$
    \Declare Source object in test scene ${o_{src}}$
    \Declare Target object in test scene ${o_{tgt}}$
    \Declare Robot's end-effector $e$
    \Declare Global accumulated constraints $C_{acc}$
    \Declare Demonstration dataset ${\cal D} = \{d_1, ..., d_n\}$
    \Declare NDF ${\cal F}$
    \Procedure{adapt-traj}{${o_{src}}, {o_{tgt}}, d, {\cal F}$}
        \State $z_{q}, \cal{Z_{\tau}}$ $\gets$ $d$
        \State $P_{o_{src}}$, $\T{{o_{src}}}{w}$ $\gets G[{o_{src}}]$
         \State $P_{o_{tgt}}$, $\T{{o_{tgt}}}{w}$ $\gets G[{o_{tgt}}]$
        \State ${\T{q_{tgt}}{o_{tgt}}} \gets \proc{ndf-optimize}({\cal F}[{o_{tgt}}], P_{o_{tgt}}, z_q)$ 
        \State\Comment{\emph{Adapt query pose to test scene based on target object}}
        \State
        \If{$l.mode {=} \texttt{detach}$}
        \State ${\T{o_{tgt}}{e}} \gets C_{acc}[\langle{o_{tgt}, e}\rangle]$
        \State\Comment{Extract required constraints from $C_{acc}$}
        \EndIf
        \State
            \For{$z^{(t)} \in {\cal Z_{\tau}}$}
                \State ${\T{q_{tgt}}{w}^{(t)}} \gets \proc{ndf-optimize}({\cal F}[{o_{src}}], P_{o_{src}}, z^{(t)})$
                \State\Comment{\emph{Adapt motion to test scene based on source object}}
                \If{$l.mode {=} \texttt{detach}$}
                    \State ${\T{e}{w}^{(t)}} \gets {\T{q_{tgt}}{w}^{(t)}}\cdot ({\T{q_{tgt}}{o_{tgt}}})^{-1}\cdot ({\T{o_{tgt}}{e}})^{-1}$
                \Else
                    \State ${\T{e}{w}^{(t)}} \gets {\T{q_{tgt}}{w}^{(t)}}$
                \EndIf
                \State \Yield{} ${\T{e}{w}^{(t)}}$ \Comment{Yield target to controller}
            \EndFor
        \State
        \If{$l.mode {=} \texttt{detach}$}
            \State delete ${C_{acc}}$[$\langle{{o_{tgt}}, e\rangle$]\Comment{Remove constraint from $C_{acc}$}
        \Else
        \State $\T{o_{src}}{o_{tgt}} \gets \T{q_{tgt}}{o_{tgt}}\cdot (\T{q_{tgt}}{w}^{(|\tau|)})^{-1}\cdot \T{o_{src}}{w}$ 
        \State\Comment{Calculate the acquired constraint at last time step}
        \State $C_{acc}[\langle{o_{src}}, {o_{tgt}}\rangle] \gets \T{o_{src}}{o_{tgt}}$ \Comment{Append constraint to $C_{acc}$}
        \EndIf
        \State
        \State $\widehat{\T{o_{tgt}}{w}} \gets \T{q_{tgt}}{w}^{(|\tau|)}\cdot (\T{q_{tgt}}{o_{tgt}})^{-1}$
        \State\Comment{Calculate the expected target object pose at last time step}
        \State
        \State $\widehat{P_{o_{tgt}}} \gets {\mathit H}^{-1}(\widehat{\T{o_{tgt}}{w}}\cdot(\T{o_{tgt}}{w})^{-1}\cdot {\mathit H}(P_{o_{tgt}}))$
        \State\Comment{Compute the expected target object point cloud, ${\mathit H}(\cdot)$ means homogeneous transformation}
        \State
        \State $G[o_{tgt}] \gets \langle\widehat{P_{o_{tgt}}}, \widehat{\T{o_{tgt}}{w}}\rangle$ \Comment{Update scene graph $G$}
    \EndProcedure
\end{algorithmic}
\end{small} % footnotesize
\end{algorithm}


==> text/Experiments.tex <==
% \section{Case Studies}
% \label{sec:exp}

% \subsection{Trajectory Adaptation to New Shapes}

% TODO

% \subsection{Goal-conditioned Skill Reasoning}

% TODO

\section{Experiments}

% \caelan{Too long}
We validate \Ours and how its components contribute to solve long-horizon tasks, perform contact-rich manipulation, and generalize to new object shapes. 

\label{sec:exp}
\subsection{Experimental Setup}

% \caelan{This is super long and not technically interesting. I would shorten. We also don't have enough numbers to justify this amount of text}

\begin{figure}
  \begin{center}
    \includegraphics[width=1\linewidth]{images/task_setup.pdf}
    \vspace{-5pt}
  \end{center}
  \caption{\textbf{Demonstration Skills and Tasks.} \textit{Top}: illustrations of demonstrated skills. \textit{Bottom}: an initial state in the five tabletop manipulation tasks we experimented on.
  }
  \label{fig:task_setup}
  \vspace{-10pt}
\end{figure}

% We compare with two state-of-the-art methods~\cite{simeonovdu2021ndf,mandlekar2023mimicgen} that share similar traits with our method and a number of ablation baselines to highlight various aspects of \Ours.

%\noindent\textbf{Tasks.}
{We compare our method to baselines (Sec.~\ref{ssec:baselines}) on two groups of challenging manipulation tasks. The first group consists of tasks from LIBERO~\cite{liu2023libero}, an existing multi-task manipulation benchmark. There, we experimented on tasks that emphasize generalization by incorporating diverse objects, spatial scene layouts, and goal configurations. Our evaluation covers the LIBERO-Spatial (10 tasks), LIBERO-Object (10 tasks), and three of the LIBERO-Long tasks. For LIBERO-Spatial tasks, we provide our system with just one demo of manipulating a bowl instance and test each system's ability to generalize over different initial bowl poses and goal configurations. For LIBERO-Object tasks, we provide our system with four demos of manipulating a cheese box, milk box, ketchup bottle, and soup can and then test our system's ability to generalize over similar objects shapes (e.g., salad dressing bottle, pudding box) and poses. To evaluate the system's long-horizon reasoning ability, we test our method on the three LIBERO-Long tasks that require manipulating multiple objects in sequence. For these tasks, we provide one additional demo of how to manipulate a mug instance.} 


\textbf{LIBERO-Spatial} - Pick up the target bowl that randomly placed on the table and put it on the plate. The benchmark includes 10 tasks with different spatial arrangements, which aim to validate generalization over spatial perturbations.  

\textbf{LIBERO-Object} - Pick up the target object that randomly placed on the table and put it into the basket. The benchmark includes 10 tasks with different target objects, which aim to test the generalization on diverse object shapes and poses.

\textbf{LIBERO-Long1} - Put both the soup can and the cheese box into the basket, with a lot of distracting objects around the target object. Given that the soup can is round and prone to slipping out of the gripper, the task is intended to assess the method's capability on long-horizon planning as well as precisely inferring the grasp pose based on the object shape.

\textbf{LIBERO-Long5} - Put the two target mugs into the two plates. Since the mugs have various shapes and poses, this long-horizon task can evaluate the method's ability on generalization over object shapes and poses.

\textbf{LIBERO-Long8} - Put both the soup can and tomato sauce can into the basket, with distracting objects densely placed around the target object. This long horizon task aims to test the method's capability on skill reusing and collision avoidance.

The second group of tasks are five new tabletop manipulation tasks (Fig.~\ref{fig:task_setup} bottom) that have greater variation in task horizon, object instances, scene layouts, goal configurations, and precision tolerances. 
%They are designed to purposefully highlight the different aspects of a generalize manipulation system. 
Four of the five tasks, MugPicking, MugInsertion, TableClear, and TableClearHard, focus on tabletop rearrangement.
For these tasks, we give each method only \textbf{two} demos, which manipulate \textbf{one} mug instance in two different ways by grasping either the handle or the rim (Fig.~\ref{fig:task_setup} top).
We test the methods' generalization over \textbf{nine} different mug shapes as well as over various poses and goal configurations. %Successfully solving the tasks requires a planner to select the skills and adapt them to the observed layout.%  1) a task of inserting the mug into the cabinet, which includes a pick skill trajectory of grasping the handle of the mug, and a place skill of inserting the mug into the cabinet; 2) a task of placing the mug into the bin, which includes a pick skill of grasping the rim, and place the mug with upright pose.
For the final ToolHang task, we provide \textbf{one} demo of how to insert the frame and hang the tool on the frame after it is assembled (Fig.~\ref{fig:task_setup} top).
%We test all methods' capability on tackling long-horizon contact-rich tasks that requires spatial generalization.

\begin{figure*}[t]
  \begin{center}
    \includegraphics[width=1\linewidth]{images/exp_vis.pdf}
    % \vspace{-5pt}
  \end{center}
  \caption{\textbf{Qualitative Visualization.} Two plans generated by \Ours, one for TableClearHard (top) and the other for ToolHang (bottom), visualized in four stages. Each row displays the planning state as a point cloud along with the planned end-effector path (upper) and snapshots of the execution process (lower).} %  \shuo{add more snapshots}
  \label{fig:exp_vis}
  \vspace{-10pt}
\end{figure*}
%\begin{itemize}
%\item 

\textbf{MugPicking} - Pick up different mugs with varying shapes and initial poses. The task tests the ability to adapt the trajectory based on object shapes and poses.

%\item 
\textbf{MugInsertion} - Insert mugs of varying shape into a tight cabinet. Both the mug and the cabinet are randomly placed on the table. This task requires fine-grained manipulation for the insertion and adaptation to different initial configurations.


%\item 
\textbf{TableClear} - This long-horizon task requires the robot to place two mugs into two bins, which aims to test the ability to achieve long-term goals by reusing the skills. % We only provide the correct picking and placing trajectory to all approaches. % since the subgoals are the same, and the robot can naively chain up the skills to complete the task without reasoning on the picking and placing strategies.

%\item 
\textbf{TableClearHard} - This long-horizon task requires the robot to stow one mug into a cabinet with side opening and place another mug into a bin. The robot must select a feasible chain of skills (side-picking to side-stowing) to transport each mug.
%and adapting the trajectories according to the observed scene.
%\end{itemize}

\textbf{ToolHang}~\cite{mandlekar2021matters} - This long-horizon task requires the robot to insert the frame into a stand with tight tolerance, and then hang the tool object on the inserted frame. The task aims to test the ability of solving low-tolerance manipulation tasks.

%  To execute the trajectory, we use a Franka Emika Panda arm controlled at 20Hz with an operational space controller (OSC). Each method is evaluated across 20 trials in each task. % The objects are randomly initialized in the scene. % \danfei{How many mug variations? Where did they come from? Mention that we used pretrained NDF on that dataset}

\subsection{Baselines} 
\label{ssec:baselines}
We compare \Ours with the three best-performing policy learning architectures on the LIBERO benchmark~\cite{liu2023libero}. Additionally, we compare with both ablation baselines and other state-of-the-art methods. Note that all NDF-based methods utilize the same NDF model~\cite{simeonovdu2021ndf}.

% \caelan{Don't need to keep citing abbreviations after they are introduced}

% \danfei{I would not put learning method here. They are not our main baselines}
%\begin{itemize}
    %\item 
    

    % \caelan{Would separate into two groups}
    
    \textbf{NDF$^{+}$}~\cite{simeonovdu2021ndf}: 
    %To ensure fair comparison, 
    We augment the original NDF manipulation planner, which only generates key-frame manipulation poses, with our task planner and the skill reasoning module, which provides the baseline with the target object and the query pose at different stages. This baseline also uses a motion planner to transition between key-frame poses. % \todo{does it use MP?}% We set up this baseline to validate the importance of trajectory for contact-rich manipulation. 
    
    %\item 
    \textbf{MimicGen$^{+}$}~\cite{mandlekar2023mimicgen}: MimicGen directly pieces together contact-rich segments from human demonstrations and linearly interpolates the intermediate steps. The robot control poses in the contact-rich segments are transformed to the relevant object frame and then sent to the controller without further adaptation. To ensure fair comparison, we augment MimicGen with a motion planner for collision avoidance. % We set up this baseline to validate the importance of adapting demonstration trajectories to test scenes based on object shapes and the relationships among objects in interaction.
    %\item \textbf{YODO}~\cite{wen2022you}:
    
    %\item 
    \textbf{Ours w/o Skill Reasoning (Ours/SR)}: This ablation removes the skill reasoning module. For each skill, we randomly choose a reference trajectory from the collected demonstrations belonging to this skill, and we bridge the intermediate transition with the motion planner. This baseline validates the importance of skill reasoning for generalizing across tasks.  
    
    %\item 
    \textbf{Ours w/o Motion Planning (Ours/MP)}: This ablation removes the motion planning component and uses linear trajectory interpolation to transition between the adapted skill trajectories generated by the optimization. We set up this baseline to validate the benefit of leveraging motion planning, a capability present in TAMP systems.
    
    %\item 
    \textbf{Naive Skill Chaining (NSC)}: This baseline ablates both the skill reasoning and the motion planning component: it randomly selects a reference trajectory for each skill, adapts the skill with NDF, and uses linear trajectory interpolation to transition between the selected trajectories. % This baseline is used to illustrate the performance when straightforwardly transferring demonstration trajectories to test scenes, without addressing the spatial transition or ensuring compatibility between different skills.

In the LIBERO benchmark, we also compare with state-of-the-art behavior cloning baselines. \textbf{RES-R} (R)~\cite{mandlekar2021matters} is a ResNet-based model with temporal encoding using LSTM. \textbf{RES-T} (T)~\cite{zhu2022viola} is a variant with transformer decoder. \textbf{ViT-T} (ViT) is a variant with Vision Transformer~\cite{kim2021vilt} encoder.
We list the reported performance in the multi-task learning setting as it is an upper bound for lifelong imitation learning~\cite{liu2023libero}. Models were trained separately for LIBERO-Spatial and LIBERO-Object, where the models for each benchmark were trained with $500$ demonstrations split across the 10 tasks. 
%We directly report the quantitative results in the original work. 
% \shuo{I think they are using different models for different benchmarks, so each model should trained with 500 demos...}

    % \textbf{RES-T}~\cite{zhu2022viola}: This model employs a ResNet-based visual backbone similar to the \textbf{RES-R} baseline but uses a transformer decoder~\cite{vaswani2017attention} as the temporal backbone for processing the ResNet output, a temporal sequence of visual tokens. The training setting is the same as the \textbf{RES-R} baseline.

    % \textbf{ViT-T}~\cite{kim2021vilt}: This baseline utilizes the ViT-T architecture, which is commonly applied in visual-language tasks. It adopts a Vision Transformer (ViT) as its visual backbone and employs a transformer decoder as its temporal backbone. The training setting is the same as the \textbf{RES-R} baseline.


\subsection{Evaluation on the LIBERO Benchmark}
% 1. sample efficiency

% \caelan{The word respectively has been used in a couple of times in a confusing manner. Usually it maps a list of things to another list of things of equal length.}\danfei{agreed }

This experiment demonstrates the performance of end-to-end learning methods versus methods that combine generalizable neural representations and model-based planners, such as \Ours and several baselines. %The LIBERO~\cite{liu2023libero} benchmark  
% To fairly compare state-of-the art policy learning approaches and other imitation learning baselines, we report our performance on the LIBERO benchmarks. We aim to highlight the exceptional sample efficiency advantage of our method. 
For the LIBERO-Spatial and LIBERO-Object tasks, the policy learning methods were trained with 500 demos.
In contrast, our system only requires namely 1 demo for LIBERO-Spatial and 4 demos for LIBERO-Object. 
For the 10 LIBERO-Spatial tasks, which emphasize generalization over diverse initial object placements, we evaluate all approaches with 5 trials for each task. 
The average success rate over 10 tasks is 84\%, which is slightly better than the 83\% success rate of T, the best multi-task learning method. For the LIBERO-Object tasks, which require generalization over object shapes and initial poses, our average success rate over the 10 tasks is 94\%, which is better than the 79\% success rate of ViT, the best policy learning method.
%by 18\% (reported as 0.79). 

We hypothesize that the performance gap is the result of differing assumed amounts of structure and object/scene representations. The policy learning methods directly learn a mapping from the scene observation to the actions and thus require a huge amount of training data to cover diverse situations. Our method, along with the action-transferring baselines (e.g., NDF, MimicGen), utilize object-centric representations to adapt the spatial correspondences from demo scenes to test scenes. MimicGen$^{+}$ assumes identical correspondences between demonstration objects and test objects, directly replaying trajectories in the local frames of test objects.
In contrast, our approach leverages learned object representations to infer spatial correspondences, enabling the transferred actions to be more robust to variations in object geometry. In contrast to NDF$^{+}$, our approach involves transferring a sequence of actions that represent each dynamic manipulation skill instead of just a single target state, in this case, the last end-effector pose in the demonstration trajectory. 
This difference enhances the effectiveness of our system to in contact-rich tasks. 
%By integrating this design with skill reasoning and motion planning, our full system becomes adept at addressing challenging long-horizon tasks that entail diverse objects, poses, and goal configurations, particularly those involving extensive contact interactions.

% \danfei{Intuition of why our method / other non-learning method works better. Make qualitative observations, e.g., common failure modes for learning methods and our methods}


\subsection{Evaluation on the Tabletop Tasks}
% 2. comp ablated versions, emph diff aspects

% We aim to emphasize different facets of our full system by quantitatively comparing \Ours with several baseline methods on the introduced tasks in Tab.~\ref{tab:compare_all}. For each task, we run 20 trials and the initial arrangement of the objects is randomly generated. 

% separate sections emph diff aspects 

\begin{figure}
% \vspace{-5pt}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{Success rates as percentages on the LIBERO benchmark tasks. MimicGen$^{+}$, Ours/MP, and Ours/SR are abbreviated as M$^{+}$, O/MP, and O/SR.}
\resizebox{1\linewidth}{!} {
\begin{tabular}{l|ccccccccc} % c|c|c|c|c|c|c|c|c
\hline
\textbf{Tasks}         & \textbf{R} & \textbf{T} & \textbf{ViT} & \textbf{NDF$^{+}$} & \textbf{MG$^{+}$} & \textbf{NSC} & \textbf{O/MP} & \textbf{O/SR} & \textbf{Ours}\\ \hline
% Spatial & 0.583  &  0.832   & 0.783  &   72   &   82   &  74  &  72   &   \textbf{86}  &  84   \\ \hline
% Object &    &  0.538   &  0.79  &  80    &   88   &   80  &  76  &  90  &  94   \\ \hline
Spatial & 58 & 83 & 78 & 72 & 82 & 74 & 72 & \textbf{86} & 84 \\ \hline
Object & 11 & 54 & 78 & 80 & 88 & 80 & 76 & 90 & \textbf{94} \\ \hline
Long1 & 0 & 20 & 8 & 50 & 40 & 10 & 10 & \textbf{70} & \textbf{70} \\ \hline
Long5 & 8 & 50 & 52 & \textbf{70} & 60 & 20 & 20 & 60 & \textbf{70} \\ \hline
Long8 & 0 & 3 & 0 & 30 & 80 & 20 & 10 & 80 & \textbf{90} \\ \hline
\end{tabular}
  }
\label{tab:compare_all_libero}
% \vspace{-5pt}
\end{figure}



\begin{figure}
% \vspace{-5pt}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{Success rates as percentages on the tabletop manipulation tasks. MimicGen$^{+}$, Ours/MP, and Ours/SR are abbreviated as M$^{+}$, O/MP, and O/SR.}
\resizebox{1\linewidth}{!} {
\begin{tabular}{l|cccccc} % l||c|c|c|c|c|c
\hline
\textbf{Tasks}            & \textbf{NDF$^{+}$} & \textbf{MG$^{+}$} & \textbf{NSC} & \textbf{O/MP} & \textbf{O/SR} & \textbf{Ours} \\ \hline
MugPicking & 80  & 70   &   \textbf{85}    &    80   &  \textbf{85}     &  \textbf{85}   \\ \hline
MugInsertion &    75   &    55    &   80    & 85  &    80   & \textbf{90} \\ \hline
TableClear &  60    &    75    &   80    &    75   &    \textbf{85}   &   \textbf{85}  \\ \hline
TableClearHard &  40   &    55  &  15   &    50 &    10 & \textbf{80} \\ \hline
ToolHang & 0 & 35 & \textbf{75} & 70 & \textbf{75} & \textbf{75} \\ \hline

\end{tabular}
  }
\label{tab:compare_all}
% \vspace{-5pt}
\end{figure}


%\caelan{How often does \Ours stitch together skills from separate demonstrations?}
% \danfei{We should also highlight that \Ours inherits the object generalization from NDF}

% \ajay{begin new results section}

% \caelan{This is a lot of text for one short table...}
%To gain deeper insights into how each component effectively tackles distinct challenges across diverse domains, 
%We conduct thorough evaluations of our approach across a spectrum of tasks that require strong generalization and reasoning capabilities, 
In the tabletop tasks, \Ours consistently achieves a high success rate (80-90\%) across all tasks and outperforms the other baselines and ablations (see Table~\ref{tab:compare_all}). 
Some qualitative results showing task execution are presented in Fig.~\ref{fig:exp_vis}.
Below, we highlight specific comparisons and takeaways that underscore the importance of the trajectory adaptation, skill planning, and motion planning components of \Ours. 

% Highlights importance of trajectory adaptation component
% \noindent\textbf{\Ours exhibits strong performance and generalization capability across short-horizon tasks.}
% The MugPicking and MugInsertion tasks are short-horizon, as they require 1 skill (pick) and 2 skills (pick and place) respectively. 
% However, unlike MugPicking, the placement in MugInsertion requires contact-rich manipulation, as it must be done precisely. We see that most baselines perform well on MugPicking (80-85\% performance with the exception of {MimicGen$^{+}$}, which gets 70\%). However, both the {NDF$^{+}$} and {MimicGen$^{+}$} baselines decrease in performance (75\% and 55\%) while \Ours maintains strong performance (90\%). This shows that \Ours enjoys generalization to a wide variety of objects from NDFs, but is able to adapt motion for contact-rich tasks using its trajectory adaptation component.
% This underscores the importance of trajectory adaptation to deal with contact-rich manipulation with novel objects, instead of simply using motion planning ({NDF$^{+}$}) or using simple replay of demonstration poses ({MimicGen$^{+}$}).

%\noindent
\textbf{\Ours exhibits strong performance across long-horizon tasks and is able to reuse skills in new contexts.}
The TableClear task requires methods to re-use the existing \textbf{two} pick-and-place human demonstrations, which only consisted of single mug and bin interactions, to stow two mugs into two bins. \Ours achieves strong performance (85\%) and outperforms {MimicGen$^{+}$} by 15\% and {NDF$^{+}$} by 25\% on this task, showcasing a superior ability to re-purposing short-horizon skill demonstrations for long-horizon manipulation.

% Highlights importance of both skill reasoning and motion planner.
%\noindent
\textbf{\Ours exhibits strong generalization capability across goals, objects, and scenes in long-horizon tasks.}
The TableClearHard task requires intelligent selection and application of different demonstration trajectories to achieve different kinds of mug placements. 
%The task also requires dealing with novel mug objects, and novel scene variations. 
Here, \Ours achieves 80\%, outperforming all other baselines by a wide margin (40\% better than {NDF$^{+}$}, 25\% better than {MimicGen$^{+}$}). 
% skill reasoning benefit
We also see the clear benefit of the skill reasoning component to achieve the different goals in this task -- \Ours outperforms (Ours/SR) by 70\% and NSC by 65\%. The omission of the skill reasoning module results in an incompatible composition of skills. For example, the robot may grip the rim of a mug and attempt to insert it into the cabinet, leading to collisions between the cabinet and the gripper. %These errors translate into a substantial deterioration in performance for both the {NSC} and Ours (-MP) baselines.
% motion planning benefit
Finally, the motion planning component is also valuable in dealing with the scene variation -- \Ours outperforms Ours/MP by 30\%. The strategy of the latter, which simply connects end-effector trajectories through linear interpolation, often leads to collisions among the robot, a held object,  and the environment. 
%In particular, we frequently observed such failures for the Ours (-MP) approach that the gripper became obstructed by the cabinet after completing the insertion of the first mug.

%\noindent
\textbf{\Ours is able to solve low-tolerance manipulation tasks.} The ToolHang task requires fine-grained manipulation skills that adapt to various object poses and contact-rich interactions. \Ours achieves 75\% success rate, outperforming {NDF$^{+}$} and {MimicGen$^{+}$} that cannot adapt their trajectories based on environment changes. Since the task does not require avoiding obstacles and reasoning over grasp poses, we observe that the ablated baselines (Ours/MP and Ours/SR) achieve similar performance as our full method.

% \noindent\textbf{Computation Efficiency Analysis}

% 3. res. presentation, time distribution


\subsection{Real-World Experiments}

% \begin{figure*}[h]
% \begin{center}
%     \includegraphics[width=1\linewidth]{images/real_res.pdf}
%     % \vspace{-5pt}
%   \end{center}
%   \caption{\textbf{Real-world Results.} Key frames of three task execution processes.}
%   \label{fig:real_res}
%   \vspace{-10pt}
% \end{figure*}

\begin{figure}[t!]
  \begin{center}
    \includegraphics[width=\linewidth]{rss24/images/real_tasks.pdf}
  \end{center}
  \caption{\textbf{Real World Tasks.} An example start and goal state for each task. The objects are initially randomly placed in a region upright on the table (details in supplementary).}
  \label{fig:real_tasks}
  \vspace{-10pt}
\end{figure}


We deploy our method on a real Franka Panda robot. The task setups are shown in Fig.~\ref{fig:real_tasks}. 
In the ``Serve Food'' task (top), the robot must place the bowl on the tray and then place the food in the bowl.
In the ``Clear Table'' task (bottom), the robot must place one target mug in the cabinet and place another mug on the tray.
The system perceives the scene with an Intel RealSense D435 camera and uses segmentation to extract the target objects. The system then transfers the perceived scene into a simulated environment to perform planning. We execute the trajectories through open-loop control. Additional results and analysis can be found in the supplementary material.


%\caelan{Analyze both of the tasks. Currently, only one is described}

% \subsection{Qualitative Evaluation}
% % 4. qualitative 
% We visualize the task execution process in Fig.~\ref{fig:exp_vis}. \shuo{explanation and analysis, failure modes analysis}


% \ajay{decide where to put below text -- better stated as a limitation (or maybe in conclusion as a place for future work to improve). Also "slipperiness" sounds very informal}
% However, it's worth noting that our system exhibits particular failure modes primarily attributable to two factors: object slipperiness and incomplete point cloud observations due to occlusion, which leads to errors in trajectory adaptation.

% \ajay{can we point to supplemental website / video to back these observations up?}
% \noindent\textbf{Other observations.} We observe that {MimicGen$^{+}$}, which essentially transforms the demonstration trajectory to align with the test object's frame without adaption, frequently fails when facing significant variations in object shape: we empirically observed that it almost never succeeded in grasping smaller mugs and often collide between the larger mug and the cabinet's bottom during testing. In contrast, for the {NDF$^{+}$} baseline, we observed that the typical failures stemmed from collisions between the mug and the cabinet. This underscores the significance of predicting a fine-grained motion trajectory rather than merely focusing on a single target pose.

% \ajay{end new results section}


%%%%% OLD RESULTS SECTION %%%%%

% \noindent\textbf{\Ours can solve long-horizon, contact-rich tasks.} 
% Our observations indicate that our approach \Ours, consistently achieves a high success rate across all tasks and surpasses the performance of all other baseline methods. The strength of \Ours lies in its ability to inherit generalization capabilities for a wide range of object shapes from NDF. Moreover, it achieves proficiency in handling long-horizon task objectives through the skill composition facilitated by the skill reasoning module. This integration of components within our method allows us to effectively address complex, long-duration tasks that involve extensive object interaction, even with diverse objects in play.

% \ajay{decide where to put below text -- better as a limitation / opportunity for future work}
% However, it's worth noting that our system exhibits particular failure modes primarily attributable to two factors: object slipperiness and incomplete point cloud observations due to occlusion, which leads to errors in trajectory adaptation.

% \noindent\textbf{Skill reasoning can form coherent plans by composing short trajectories.} Our findings emphasize the critical importance of the skill reasoning component in solving long-horizon tasks that necessitate a blend of picking and placing strategies. In the case of the TableClearHard task, the omission of the skill reasoning module results in an incompatible composition of skills. For example, the robot may opt to grip the rim of a mug and attempt to insert it into the cabinet, leading to collisions between the cabinet and the gripper. These errors translate into a substantial deterioration in performance for both the {NSC} and Ours (-MP) baselines.

% \noindent\textbf{Integrating motion planner enables cross-layout generalization.} We observe that for TableClear and TableClearHard, which require manipulating multiple objects and long spatial transitions between successive skills, it is important to bridge the transition with motion planning. Simply connecting end-effector trajectories through linear interpolation without considering environmental obstacles often leads to collisions between the robot or the held object and its surroundings. In particular, we frequently observed such failures in the case of the Ours (-MP) approach when performing the TableClearHard task, where the gripper became obstructed by the cabinet after completing the insertion of the first mug.

% \ajay{can we point to supplemental website / video to back these observations up?}
% \noindent\textbf{Other observations.} We observe that {MimicGen$^{+}$}, which essentially transforms the demonstration trajectory to align with the test object's frame without adaption, frequently fails when facing significant variations in object shape: we empirically observed that it almost never succeeded in grasping smaller mugs and often collide between the larger mug and the cabinet's bottom during testing. In contrast, for the {NDF$^{+}$} baseline, we observed that the typical failures stemmed from collisions between the mug and the cabinet. This underscores the significance of predicting a fine-grained motion trajectory rather than merely focusing on a single target pose.

%%%%% OLD RESULTS SECTION END %%%%%

% \subsection{Qualitative Analysis}







% \caelan{Would remove this subsection but keep the figure.}

% We present a visual representation of various aspects of our full system, including the generated trajectories at different stages and the reconstructed scene state represented as a point cloud captured at the outset of the task in Fig.~\ref{fig:exp_vis}. We further illustrate the execution of these trajectories through a series of snapshots.

% A notable observation is the pivotal role played by the motion planning component, which enables the robot to navigate through the cluttered scene while avoiding collisions. Additionally, the trajectory adaptation module proves its precision by adeptly transforming the demonstration trajectories to align with the specifics of the test scenes.

% \subsection{Real-world Evaluations}

% \todo{show snapshots of real world execution, report successful trials}




==> text/Experiments_revised.tex <==
% \section{Case Studies}
% \label{sec:exp}

% \subsection{Trajectory Adaptation to New Shapes}

% TODO

% \subsection{Goal-conditioned Skill Reasoning}

% TODO

\section{Experiments}

% \caelan{Too long}
We validate \Ours and how its components contribute to solve long-horizon tasks, perform {fine-grained} manipulation, and generalize to new object shapes. 

\label{sec:exp}
\subsection{Experimental Setup}

% \caelan{This is super long and not technically interesting. I would shorten. We also don't have enough numbers to justify this amount of text}


% We compare with two state-of-the-art methods~\cite{simeonovdu2021ndf,mandlekar2023mimicgen} that share similar traits with our method and a number of ablation baselines to highlight various aspects of \Ours.

%\noindent\textbf{Tasks.}
{We compare our method to baselines (Sec.~\ref{ssec:baselines}) on two groups of challenging manipulation tasks. The first group consists of tasks from LIBERO~\cite{liu2023libero}, an existing multi-task manipulation benchmark. Our evaluation covers the LIBERO-Spatial (10 tasks), LIBERO-Object (10 tasks), and three of the LIBERO-Long tasks. For LIBERO-Spatial tasks, we provide our system with just one demo of manipulating a bowl instance and test each system's ability to generalize over different initial bowl poses and goal configurations. For LIBERO-Object tasks, we provide our system with four demos of manipulating a cheese box, milk box, ketchup bottle, and soup can and then test our system's ability to generalize over similar objects shapes (e.g., salad dressing bottle, pudding box) and poses. To evaluate the system's long-horizon reasoning ability, we test our method on the three LIBERO-Long tasks that require manipulating multiple objects in sequence. For these tasks, we provide one additional demo of how to manipulate a mug instance.} 


\textbf{LIBERO-Spatial} - Pick up the target bowl and place it on the goal plate. The benchmark includes 10 tasks with different spatial arrangements to validate generalization over spatial perturbations.

\textbf{LIBERO-Object} - Pick up the target object put it into the basket. The benchmark includes 10 tasks with different target objects to test the generalization on diverse object shapes and poses.

\textbf{LIBERO-Long1} - Put both the soup can and the cheese box into the basket, with a lot of distracting objects around the target object. Given that the soup can is round and prone to slipping out of the gripper, the task is intended to assess the method's capability on long-horizon planning as well as precisely inferring the grasp pose based on the object shape.

\textbf{LIBERO-Long5} - Put the two target mugs into the two plates. Since the mugs have various shapes and poses, this long-horizon task can evaluate the method's ability on generalization over object shapes and poses.

\textbf{LIBERO-Long8} - Put both the soup can and tomato sauce can into the basket, with distracting objects densely placed around the target object. This long horizon task aims to test the method's capability on skill reusing and collision avoidance.

\begin{wrapfigure}{r}{.5\textwidth}
  \centering
    \includegraphics[width=1\linewidth]{images/task_setup.pdf}
    \vspace{-5pt}
  \caption{\textbf{Demonstration Skills and Tasks.} \textit{Top}: illustrations of demonstrated skills. \textit{Bottom}: an initial state in the five tabletop manipulation tasks we experimented on.
  }
  \label{fig:task_setup}
  % \vspace{-10pt}
\end{wrapfigure}


The second group of tasks are five new tabletop manipulation tasks (Fig.~\ref{fig:task_setup} bottom) that have greater variation in task horizon, object instances, scene layouts, goal configurations, and precision tolerances. 
%They are designed to purposefully highlight the different aspects of a generalize manipulation system. 
Four of the five tasks, MugPicking, MugInsertion, TableClear, and TableClearHard, focus on tabletop rearrangement.
For these tasks, we give each method only \textbf{two} demos, which manipulate \textbf{one} mug instance in two different ways by grasping either the handle or the rim (Fig.~\ref{fig:task_setup} top).
We test the methods' generalization over \textbf{nine} different mug shapes as well as over various poses and goal configurations. %Successfully solving the tasks requires a planner to select the skills and adapt them to the observed layout.%  1) a task of inserting the mug into the cabinet, which includes a pick skill trajectory of grasping the handle of the mug, and a place skill of inserting the mug into the cabinet; 2) a task of placing the mug into the bin, which includes a pick skill of grasping the rim, and place the mug with upright pose.
For the final ToolHang task, we provide \textbf{one} demo of how to insert the frame and hang the tool on the frame after it is assembled (Fig.~\ref{fig:task_setup} top).
%We test all methods' capability on tackling long-horizon contact-rich tasks that requires spatial generalization.

% \begin{figure*}[t]
%   \begin{center}
%     \includegraphics[width=0.9\linewidth]{images/exp_vis.pdf}
%     % \vspace{-5pt}
%   \end{center}
%   \caption{\textbf{Qualitative Visualization.} Two plans generated by \Ours, one for TableClearHard (top) and the other for ToolHang (bottom), visualized in four stages. Each row displays the planning state as a point cloud along with the planned end-effector path (upper) and snapshots of the execution process (lower).} %  \shuo{add more snapshots}
%   \label{fig:exp_vis}
%   \vspace{-10pt}
% \end{figure*}
%\begin{itemize}
%\item 

\textbf{MugPicking} - Pick up different mugs with varying shapes and initial poses. The task tests the ability to adapt the trajectory based on object shapes and poses.

%\item 
\textbf{MugInsertion} - Insert mugs of varying shape into a tight cabinet. Both the mug and the cabinet are randomly placed on the table. This task requires fine-grained manipulation for the insertion and adaptation to different initial configurations.


%\item 
\textbf{TableClear} - This long-horizon task requires the robot to place two mugs into two bins, which aims to test the ability to achieve long-term goals by reusing the skills. % We only provide the correct picking and placing trajectory to all approaches. % since the subgoals are the same, and the robot can naively chain up the skills to complete the task without reasoning on the picking and placing strategies.

%\item 
\textbf{TableClearHard} - This long-horizon task requires the robot to stow one mug into a cabinet with side opening and place another mug into a bin. The robot must select a feasible chain of skills (side-picking to side-stowing) to transport each mug.
%and adapting the trajectories according to the observed scene.
%\end{itemize}

\textbf{ToolHang}~\cite{mandlekar2021matters} - This long-horizon task requires the robot to insert the frame into a stand with tight tolerance, and then hang the tool object on the inserted frame. The task aims to test the ability of solving low-tolerance manipulation tasks.

%  To execute the trajectory, we use a Franka Emika Panda arm controlled at 20Hz with an operational space controller (OSC). Each method is evaluated across 20 trials in each task. % The objects are randomly initialized in the scene. % \danfei{How many mug variations? Where did they come from? Mention that we used pretrained NDF on that dataset}

\subsection{Baselines} 
\label{ssec:baselines}
We compare \Ours with the three best-performing policy learning architectures on the LIBERO benchmark~\cite{liu2023libero}. Additionally, we compare with both ablation baselines and other state-of-the-art methods. Note that all NDF-based methods utilize the same NDF model~\cite{simeonovdu2021ndf}.

% \caelan{Don't need to keep citing abbreviations after they are introduced}

% \danfei{I would not put learning method here. They are not our main baselines}
%\begin{itemize}
    %\item 
    

    % \caelan{Would separate into two groups}
    
    \textbf{NDF$^{+}$}~\cite{simeonovdu2021ndf}: 
    %To ensure fair comparison, 
    We augment the original NDF manipulation planner, which only generates key-frame manipulation poses, with our task planner and the skill reasoning module, which provides the baseline with the target object and the query pose at different stages. This baseline also uses a motion planner to transition between key-frame poses. % \todo{does it use MP?}% We set up this baseline to validate the importance of trajectory for contact-rich manipulation. 
    
    %\item 
    \textbf{MimicGen$^{+}$}~\cite{mandlekar2023mimicgen}: MimicGen directly pieces together segments from human demonstrations that require high-precision motion and linearly interpolates the intermediate steps. The robot control poses in these segments are transformed to the relevant object frame and then sent to the controller without further adaptation. To ensure fair comparison, we augment MimicGen with a motion planner for collision avoidance. % We set up this baseline to validate the importance of adapting demonstration trajectories to test scenes based on object shapes and the relationships among objects in interaction.
    %\item \textbf{YODO}~\cite{wen2022you}:
    
    %\item 
    \textbf{Ours w/o Skill Reasoning (Ours/SR)}: This ablation removes the skill reasoning module. For each skill, we randomly choose a reference trajectory from the collected demonstrations belonging to this skill, and we bridge the intermediate transition with the motion planner. This baseline validates the importance of skill reasoning for generalizing across tasks.  
    
    %\item 
    \textbf{Ours w/o Motion Planning (Ours/MP)}: This ablation removes the motion planning component and uses linear trajectory interpolation to transition between the adapted skill trajectories generated by the optimization. We set up this baseline to validate the benefit of leveraging motion planning, a capability present in TAMP systems.
    
    %\item 
    \textbf{Naive Skill Chaining (NSC)}: This baseline ablates both the skill reasoning and the motion planning component: it randomly selects a reference trajectory for each skill, adapts the skill with NDF, and uses linear trajectory interpolation to transition between the selected trajectories. % This baseline is used to illustrate the performance when straightforwardly transferring demonstration trajectories to test scenes, without addressing the spatial transition or ensuring compatibility between different skills.

In the LIBERO benchmark, we also compare with state-of-the-art behavior cloning baselines. \textbf{RES-R} (R)~\cite{mandlekar2021matters} is a ResNet-based model with temporal encoding using LSTM. \textbf{RES-T} (T)~\cite{zhu2022viola} is a variant with transformer decoder. \textbf{ViT-T} (ViT) is a variant with Vision Transformer~\cite{kim2021vilt} encoder.
We list the reported performance in the multi-task learning setting as it is an upper bound for lifelong imitation learning~\cite{liu2023libero}. Models were trained separately for LIBERO-Spatial and LIBERO-Object, where the models for each benchmark were trained with $500$ demonstrations split across the 10 tasks. 
%We directly report the quantitative results in the original work. 
% \shuo{I think they are using different models for different benchmarks, so each model should trained with 500 demos...}

    % \textbf{RES-T}~\cite{zhu2022viola}: This model employs a ResNet-based visual backbone similar to the \textbf{RES-R} baseline but uses a transformer decoder~\cite{vaswani2017attention} as the temporal backbone for processing the ResNet output, a temporal sequence of visual tokens. The training setting is the same as the \textbf{RES-R} baseline.

    % \textbf{ViT-T}~\cite{kim2021vilt}: This baseline utilizes the ViT-T architecture, which is commonly applied in visual-language tasks. It adopts a Vision Transformer (ViT) as its visual backbone and employs a transformer decoder as its temporal backbone. The training setting is the same as the \textbf{RES-R} baseline.


\subsection{Evaluation on the LIBERO Benchmark}
% 1. sample efficiency

% \caelan{The word respectively has been used in a couple of times in a confusing manner. Usually it maps a list of things to another list of things of equal length.}\danfei{agreed }

This experiment demonstrates the performance of end-to-end learning methods versus methods that combine generalizable neural representations and model-based planners, such as \Ours and several baselines. %The LIBERO~\cite{liu2023libero} benchmark  
% To fairly compare state-of-the art policy learning approaches and other imitation learning baselines, we report our performance on the LIBERO benchmarks. We aim to highlight the exceptional sample efficiency advantage of our method. 
For the LIBERO-Spatial and LIBERO-Object tasks, the policy learning methods were trained with 500 demos.
In contrast, our system only requires namely 1 demo for LIBERO-Spatial and 4 demos for LIBERO-Object. 
For the 10 LIBERO-Spatial tasks, which emphasize generalization over diverse initial object placements, we evaluate all approaches with 5 trials for each task. 
The average success rate over 10 tasks is 84\%, which is slightly better than the 83\% success rate of T, the best multi-task learning method. For the LIBERO-Object tasks, which require generalization over object shapes and initial poses, our average success rate over the 10 tasks is 94\%, which is better than the 79\% success rate of ViT, the best policy learning method.
%by 18\% (reported as 0.79). 


\begin{wrapfigure}{l}{.6\textwidth}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{Success rates as percentages on the LIBERO benchmark tasks. MimicGen$^{+}$, Ours/MP, and Ours/SR are abbreviated as M$^{+}$, O/MP, and O/SR.}
\resizebox{1\linewidth}{!} {
\begin{tabular}{l|ccccccccc} % c|c|c|c|c|c|c|c|c
\hline
\textbf{Tasks}         & \textbf{R} & \textbf{T} & \textbf{ViT} & \textbf{NDF$^{+}$} & \textbf{MG$^{+}$} & \textbf{NSC} & \textbf{O/MP} & \textbf{O/SR} & \textbf{Ours}\\ \hline
% Spatial & 0.583  &  0.832   & 0.783  &   72   &   82   &  74  &  72   &   \textbf{86}  &  84   \\ \hline
% Object &    &  0.538   &  0.79  &  80    &   88   &   80  &  76  &  90  &  94   \\ \hline
Spatial & 58 & 83 & 78 & 72 & 82 & 74 & 72 & \textbf{86} & 84 \\ \hline
Object & 11 & 54 & 78 & 80 & 88 & 80 & 76 & 90 & \textbf{94} \\ \hline
Long1 & 0 & 20 & 8 & 50 & 40 & 10 & 10 & \textbf{70} & \textbf{70} \\ \hline
Long5 & 8 & 50 & 52 & \textbf{70} & 60 & 20 & 20 & 60 & \textbf{70} \\ \hline
Long8 & 0 & 3 & 0 & 30 & 80 & 20 & 10 & 80 & \textbf{90} \\ \hline
\end{tabular}
  }
\label{tab:compare_all_libero}
\end{wrapfigure}


We hypothesize that the performance gap is the result of differing assumed amounts of structure and object/scene representations. The policy learning methods directly learn a mapping from the scene observation to the actions and thus require a huge amount of training data to cover diverse situations. Our method, along with the action-transferring baselines (e.g., NDF, MimicGen), utilize object-centric representations to adapt the spatial correspondences from demo scenes to test scenes. MimicGen$^{+}$ assumes identical correspondences between demonstration objects and test objects, directly replaying trajectories in the local frames of test objects.

In contrast, our approach leverages learned object representations to infer spatial correspondences, enabling the transferred actions to be more robust to variations in object geometry. In contrast to NDF$^{+}$, our approach involves transferring a sequence of actions that represent each dynamic manipulation skill instead of just a single target state, in this case, the last end-effector pose in the demonstration trajectory. 
This difference enhances the effectiveness of our system to in fine-grained manipulation tasks. 
%By integrating this design with skill reasoning and motion planning, our full system becomes adept at addressing challenging long-horizon tasks that entail diverse objects, poses, and goal configurations, particularly those involving extensive contact interactions.

% \danfei{Intuition of why our method / other non-learning method works better. Make qualitative observations, e.g., common failure modes for learning methods and our methods}


\subsection{Evaluation on the Tabletop Tasks}
% 2. comp ablated versions, emph diff aspects

% We aim to emphasize different facets of our full system by quantitatively comparing \Ours with several baseline methods on the introduced tasks in Tab.~\ref{tab:compare_all}. For each task, we run 20 trials and the initial arrangement of the objects is randomly generated. 

% separate sections emph diff aspects 



% \begin{figure}
% % \vspace{-5pt}
% \makeatletter\def\@captype{table}\makeatother% "Change float to table"
% \caption{Success rates as percentages on the LIBERO benchmark tasks. MimicGen$^{+}$, Ours/MP, and Ours/SR are abbreviated as M$^{+}$, O/MP, and O/SR.}
% \resizebox{1\linewidth}{!} {
% \begin{tabular}{l|ccccccccc} % c|c|c|c|c|c|c|c|c
% \hline
% \textbf{Tasks}         & \textbf{R} & \textbf{T} & \textbf{ViT} & \textbf{NDF$^{+}$} & \textbf{MG$^{+}$} & \textbf{NSC} & \textbf{O/MP} & \textbf{O/SR} & \textbf{Ours}\\ \hline
% % Spatial & 0.583  &  0.832   & 0.783  &   72   &   82   &  74  &  72   &   \textbf{86}  &  84   \\ \hline
% % Object &    &  0.538   &  0.79  &  80    &   88   &   80  &  76  &  90  &  94   \\ \hline
% Spatial & 58 & 83 & 78 & 72 & 82 & 74 & 72 & \textbf{86} & 84 \\ \hline
% Object & 11 & 54 & 78 & 80 & 88 & 80 & 76 & 90 & \textbf{94} \\ \hline
% Long1 & 0 & 20 & 8 & 50 & 40 & 10 & 10 & \textbf{70} & \textbf{70} \\ \hline
% Long5 & 8 & 50 & 52 & \textbf{70} & 60 & 20 & 20 & 60 & \textbf{70} \\ \hline
% Long8 & 0 & 3 & 0 & 30 & 80 & 20 & 10 & 80 & \textbf{90} \\ \hline
% \end{tabular}
%   }
% \label{tab:compare_all_libero}
% % \vspace{-5pt}
% \end{figure}


%\caelan{How often does \Ours stitch together skills from separate demonstrations?}
% \danfei{We should also highlight that \Ours inherits the object generalization from NDF}

% \ajay{begin new results section}

% \caelan{This is a lot of text for one short table...}
%To gain deeper insights into how each component effectively tackles distinct challenges across diverse domains, 
%We conduct thorough evaluations of our approach across a spectrum of tasks that require strong generalization and reasoning capabilities, 
In the tabletop tasks, \Ours consistently achieves a high success rate (80-90\%) across all tasks and outperforms the other baselines and ablations (see Table~\ref{tab:compare_all}). 
Some qualitative results showing task execution are presented in Fig.~\ref{fig:exp_vis}.

Below, we highlight specific comparisons and takeaways that underscore the importance of the trajectory adaptation, skill planning, and motion planning components of \Ours. 

% Highlights importance of trajectory adaptation component
% \noindent\textbf{\Ours exhibits strong performance and generalization capability across short-horizon tasks.}
% The MugPicking and MugInsertion tasks are short-horizon, as they require 1 skill (pick) and 2 skills (pick and place) respectively. 
% However, unlike MugPicking, the placement in MugInsertion requires contact-rich manipulation, as it must be done precisely. We see that most baselines perform well on MugPicking (80-85\% performance with the exception of {MimicGen$^{+}$}, which gets 70\%). However, both the {NDF$^{+}$} and {MimicGen$^{+}$} baselines decrease in performance (75\% and 55\%) while \Ours maintains strong performance (90\%). This shows that \Ours enjoys generalization to a wide variety of objects from NDFs, but is able to adapt motion for contact-rich tasks using its trajectory adaptation component.
% This underscores the importance of trajectory adaptation to deal with contact-rich manipulation with novel objects, instead of simply using motion planning ({NDF$^{+}$}) or using simple replay of demonstration poses ({MimicGen$^{+}$}).

\begin{wrapfigure}{r}{.5\textwidth}
% \vspace{-5pt}
\makeatletter\def\@captype{table}\makeatother% "Change float to table"
\caption{Success rates as percentages on the tabletop manipulation tasks. MimicGen$^{+}$, Ours/MP, and Ours/SR are abbreviated as M$^{+}$, O/MP, and O/SR.}
\resizebox{1\linewidth}{!} {
\begin{tabular}{l|cccccc} % l||c|c|c|c|c|c
\hline
\textbf{Tasks}            & \textbf{NDF$^{+}$} & \textbf{MG$^{+}$} & \textbf{NSC} & \textbf{O/MP} & \textbf{O/SR} & \textbf{Ours} \\ \hline
MugPicking & 80  & 70   &   \textbf{85}    &    80   &  \textbf{85}     &  \textbf{85}   \\ \hline
MugInsertion &    75   &    55    &   80    & 85  &    80   & \textbf{90} \\ \hline
TableClear &  60    &    75    &   80    &    75   &    \textbf{85}   &   \textbf{85}  \\ \hline
TableClearHard &  40   &    55  &  15   &    50 &    10 & \textbf{80} \\ \hline
ToolHang & 0 & 35 & \textbf{75} & 70 & \textbf{75} & \textbf{75} \\ \hline

\end{tabular}
  }
\label{tab:compare_all}
% \vspace{-5pt}
\end{wrapfigure}


%\noindent
\textbf{\Ours exhibits strong performance across long-horizon tasks and is able to reuse skills in new contexts.}
The TableClear task requires methods to re-use the existing \textbf{two} pick-and-place human demonstrations, which only consisted of single mug and bin interactions, to stow two mugs into two bins. \Ours achieves strong performance (85\%) and outperforms {MimicGen$^{+}$} by 15\% and {NDF$^{+}$} by 25\% on this task, showcasing a superior ability to re-purposing short-horizon skill demonstrations for long-horizon manipulation.

% Highlights importance of both skill reasoning and motion planner.
%\noindent
\textbf{\Ours exhibits strong generalization capability across goals, objects, and scenes in long-horizon tasks.}
The TableClearHard task requires intelligent selection and application of different demonstration trajectories to achieve different kinds of mug placements. 
%The task also requires dealing with novel mug objects, and novel scene variations. 
Here, \Ours achieves 80\%, outperforming all other baselines by a wide margin (40\% better than {NDF$^{+}$}, 25\% better than {MimicGen$^{+}$}). 
% skill reasoning benefit
We also see the clear benefit of the skill reasoning component to achieve the different goals in this task -- \Ours outperforms (Ours/SR) by 70\% and NSC by 65\%. The omission of the skill reasoning module results in an incompatible composition of skills. For example, the robot may grip the rim of a mug and attempt to insert it into the cabinet, leading to collisions between the cabinet and the gripper. %These errors translate into a substantial deterioration in performance for both the {NSC} and Ours (-MP) baselines.
% motion planning benefit
Finally, the motion planning component is also valuable in dealing with the scene variation -- \Ours outperforms Ours/MP by 30\%. The strategy of the latter, which simply connects end-effector trajectories through linear interpolation, often leads to collisions among the robot, a held object,  and the environment. 
%In particular, we frequently observed such failures for the Ours (-MP) approach that the gripper became obstructed by the cabinet after completing the insertion of the first mug.

%\noindent
\textbf{\Ours is able to solve low-tolerance manipulation tasks.} The ToolHang task requires fine-grained manipulation skills that adapt to various object poses. \Ours achieves 75\% success rate, outperforming {NDF$^{+}$} and {MimicGen$^{+}$} that cannot adapt their trajectories based on environment changes. Since the task does not require avoiding obstacles and reasoning over grasp poses, we observe that the ablated baselines (Ours/MP and Ours/SR) achieve similar performance as our full method.

% \noindent\textbf{Computation Efficiency Analysis}

% 3. res. presentation, time distribution


\subsection{Real-World Experiments}\label{sec:real_exp}

% \begin{figure*}[h]
% \begin{center}
%     \includegraphics[width=1\linewidth]{images/real_res.pdf}
%     % \vspace{-5pt}
%   \end{center}
%   \caption{\textbf{Real-world Results.} Key frames of three task execution processes.}
%   \label{fig:real_res}
%   \vspace{-10pt}
% \end{figure*}



{
We deploy \Ours on a real Franka Panda robot. The task setups are shown in Fig.~\ref{fig:real_tasks}. Here we briefly describe each task:

\textbf{Sort Tableware} - Insert a dish into a narrow slot on the rack and stack two bowls on top of it.

\textbf{Make Coffee} - Place a mug under the coffee machine, insert a coffee pod into a tight holder, close the lid and then press the button.

\textbf{Insert Screwdriver} - Insert a screwdriver into a tight slot on the storage rack.

\textbf{Use Tool} - Grasp the L-shape tool to poke and hook two boxes, and stack them. This task is inspired by~\cite{loula2020task, toussaint2018differentiable, xu2021deep}. 

\textbf{Clear Mugs (Same Goal)} - Hang two mugs on the mug tree.

\textbf{Clear Mugs (Multi Goal)} - Hang one mug on the mug tree, and insert another mug into the cabinet.


% In the ``Sort Tableware'' task (top), the robot must insert a dish into a narrow slot on the rack and stack two bowls on top of it. This task spans multiple stages, each involving changes in system kinematics such as attaching or detaching objects. In the ``Make Coffee'' task (bottom), the robot is required to place a mug in the correct position under the coffee machine, pick and insert a coffee pod into a tight holder, close the lid of the machine, and then press the button. Similar to the previous task, this also entails multiple stages and involves manipulation with rich contact interactions.

We use a Microsoft Azure Kinect camera for scene perception, the camera is mounted in front of the robot and calibrated. We leverage SAM~\cite{kirillov2023segany} for target object segmentation. \Ours plans trajectories directly from real-world perception results and executes them via open-loop control. \Ours achieves a 60\% success rate on the ``Make Coffee'' task, 70\% success rate on the ``Insert Screwdriver'' task, 90\% success rate on the ``Sort Tableware'' and ``Use Tool'' tasks, and 80\% success rate on the ``Clear Mugs (Same Goal)'' and ``Clear Mugs (Multi Goal)'' tasks. Additional results and analysis are provided in the supplementary material.}

% \begin{wrapfigure}{l}{.5\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/real_task_setup_v2.pdf}
%   \caption{\textbf{Real-world Tasks.} 
%   {An example of the initial state and a goal state for each of the tasks (left), and the reset ranges visualized as an overlay of the initial state in each trial (right). See the supplementary material for more details.}}
%   \label{fig:real_tasks}
%   % \vspace{-10pt}
% \end{wrapfigure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/real_task_setup_v2.pdf}
    \caption{\textbf{Real-world Tasks.} 
  {An example of the initial state and a goal state for each of the tasks, and the reset ranges visualized as an overlay of the initial state in each trial. See the supplementary material for more details.}}
  \label{fig:real_tasks}
\end{figure}


% \begin{wrapfigure}{l}{.5\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/real_task_setup.pdf}
%   \caption{\textbf{Real-world Tasks.} 
%   {An example of the initial state and a goal state for each of the tasks (left), and the reset ranges visualized as an overlay of the initial state in each trial (right). See the supplementary material for more details.}}
%   \label{fig:real_tasks}
%   % \vspace{-10pt}
% \end{wrapfigure}



%\caelan{Analyze both of the tasks. Currently, only one is described}

% \subsection{Qualitative Evaluation}
% % 4. qualitative 
% We visualize the task execution process in Fig.~\ref{fig:exp_vis}. \shuo{explanation and analysis, failure modes analysis}


% \ajay{decide where to put below text -- better stated as a limitation (or maybe in conclusion as a place for future work to improve). Also "slipperiness" sounds very informal}
% However, it's worth noting that our system exhibits particular failure modes primarily attributable to two factors: object slipperiness and incomplete point cloud observations due to occlusion, which leads to errors in trajectory adaptation.

% \ajay{can we point to supplemental website / video to back these observations up?}
% \noindent\textbf{Other observations.} We observe that {MimicGen$^{+}$}, which essentially transforms the demonstration trajectory to align with the test object's frame without adaption, frequently fails when facing significant variations in object shape: we empirically observed that it almost never succeeded in grasping smaller mugs and often collide between the larger mug and the cabinet's bottom during testing. In contrast, for the {NDF$^{+}$} baseline, we observed that the typical failures stemmed from collisions between the mug and the cabinet. This underscores the significance of predicting a fine-grained motion trajectory rather than merely focusing on a single target pose.

% \ajay{end new results section}


%%%%% OLD RESULTS SECTION %%%%%

% \noindent\textbf{\Ours can solve long-horizon, contact-rich tasks.} 
% Our observations indicate that our approach \Ours, consistently achieves a high success rate across all tasks and surpasses the performance of all other baseline methods. The strength of \Ours lies in its ability to inherit generalization capabilities for a wide range of object shapes from NDF. Moreover, it achieves proficiency in handling long-horizon task objectives through the skill composition facilitated by the skill reasoning module. This integration of components within our method allows us to effectively address complex, long-duration tasks that involve extensive object interaction, even with diverse objects in play.

% \ajay{decide where to put below text -- better as a limitation / opportunity for future work}
% However, it's worth noting that our system exhibits particular failure modes primarily attributable to two factors: object slipperiness and incomplete point cloud observations due to occlusion, which leads to errors in trajectory adaptation.

% \noindent\textbf{Skill reasoning can form coherent plans by composing short trajectories.} Our findings emphasize the critical importance of the skill reasoning component in solving long-horizon tasks that necessitate a blend of picking and placing strategies. In the case of the TableClearHard task, the omission of the skill reasoning module results in an incompatible composition of skills. For example, the robot may opt to grip the rim of a mug and attempt to insert it into the cabinet, leading to collisions between the cabinet and the gripper. These errors translate into a substantial deterioration in performance for both the {NSC} and Ours (-MP) baselines.

% \noindent\textbf{Integrating motion planner enables cross-layout generalization.} We observe that for TableClear and TableClearHard, which require manipulating multiple objects and long spatial transitions between successive skills, it is important to bridge the transition with motion planning. Simply connecting end-effector trajectories through linear interpolation without considering environmental obstacles often leads to collisions between the robot or the held object and its surroundings. In particular, we frequently observed such failures in the case of the Ours (-MP) approach when performing the TableClearHard task, where the gripper became obstructed by the cabinet after completing the insertion of the first mug.

% \ajay{can we point to supplemental website / video to back these observations up?}
% \noindent\textbf{Other observations.} We observe that {MimicGen$^{+}$}, which essentially transforms the demonstration trajectory to align with the test object's frame without adaption, frequently fails when facing significant variations in object shape: we empirically observed that it almost never succeeded in grasping smaller mugs and often collide between the larger mug and the cabinet's bottom during testing. In contrast, for the {NDF$^{+}$} baseline, we observed that the typical failures stemmed from collisions between the mug and the cabinet. This underscores the significance of predicting a fine-grained motion trajectory rather than merely focusing on a single target pose.

%%%%% OLD RESULTS SECTION END %%%%%

% \subsection{Qualitative Analysis}







% \caelan{Would remove this subsection but keep the figure.}

% We present a visual representation of various aspects of our full system, including the generated trajectories at different stages and the reconstructed scene state represented as a point cloud captured at the outset of the task in Fig.~\ref{fig:exp_vis}. We further illustrate the execution of these trajectories through a series of snapshots.

% A notable observation is the pivotal role played by the motion planning component, which enables the robot to navigate through the cluttered scene while avoiding collisions. Additionally, the trajectory adaptation module proves its precision by adeptly transforming the demonstration trajectories to align with the specifics of the test scenes.

% \subsection{Real-world Evaluations}

% \todo{show snapshots of real world execution, report successful trials}




==> text/Method.tex <==
%\section{Background and Prerequisites}
\section{Problem Formulation}
%\section{Few-shot Manipulation for Unknown Objects}
\label{sec:method}
% introducing the problem formulation, the concept of our framework, the input and output of our system, the requirements and conditions for implementing the system, and the scenarios and advantages of the framework.

%\todo{Problem formulation, concept, requirements for inputs/observations, outputs, advantages (handling novel unknown objects, acquisition of new skills with few demonstrations, easy to support continuous skill integration)}

We seek to apply NDFs~\cite{sundermeyer2021contact}, a type of Neural Object Descriptor, to robot manipulation. First, we review background on NDF for category-consistent frame estimation (Section~\ref{sec:ndf}).
Then, we describe our problem setting (Section~\ref{sec:problem}).

\subsection{Neural Descriptor Fields (NDF)} \label{sec:ndf}
%\caelan{Appears to be a subset of "Problem Formulation"}

NDF~\cite{simeonovdu2021ndf} were first proposed for category-invariant modeling of object rigid transformations. 
A NDF model $\posendf(T \mid P)$ takes in an object shape that is represented as a point cloud $P \in \mathbb{R}^{N\times3}$ and a set of query positions $\{R \cdot x_i+t \mid x_i \in X\}$.
Let $T = [R \mid t] \in \SE{3}$ be a rigid transformation and $X \in \mathbb{R}^{M\times3}$ be a vector of query points.
The NDF outputs features corresponding to the query points:
\begin{equation*}
z \gets \posendf(T \mid P) \equiv \bigoplus_{x_i \in X} \pointndf(R \cdot x_i+t \mid P).
\label{eq:pose_enc}
\end{equation*}

A key advantage of NDF features is that they are only related to the queries in the object's local frame, therefore a rigid transformation $R \in \SE{3}$ applied to both the shape and the query pose has no affect on the feature:
%would affect the extracted feature, which allows us to generalize the extracted pose $R \cdot T$ with arbitrary configuration $R$ of the new shape:
\begin{equation*}
\posendf(R \cdot T \mid R \cdot P) = \posendf(T \mid P).
\label{eq:pose_enc}
\end{equation*}

NDFs are typically used to solve an inverse problem: recover a transformation $T$ that corresponds to a query feature $z$.
This can be framed as the following optimization problem and solved by 1) randomly initializing the transform, 2) backpropgating to compute the error gradient, and 3) iteratively moving along the gradient to minimize the error:
\begin{equation*}
% \proc{ndf-optimize}(P, \posedescriptor) \equiv \underset{T}{\text{argmin}} ||\posedescriptor -  \posendf(T \mid P)||_1
\proc{ndf-optimize}(F, P, z) \equiv \underset{T}{\text{argmin}} ||z -  \posendf(T \mid P)||. % _1
\end{equation*}

%Given a reference pose $T$ and a reference object $P$, we can first obtain the corresponding feature $z$. 
%To obtain the new pose $T'$ that maps points from the base frame to the geometric equivalent positions in the new shape's frame, we can randomly initialize the new pose and back-propagate the gradient to it: 

% \begin{equation*}
% T' = \underset{T'}{\text{argmin}} ||z - \posendf(T' \mid P')||.
% \label{eq:pose_enc}
% \end{equation*}
%Let the following solve for a transformation $T$ that matches NDF feature $z$:

\subsection{Problem Setting} \label{sec:problem}

% MimicGen: A Data Generation System for Scalable Robot Learning using Human Demonstrations
% https://openreview.net/forum?id=dk-2R1f_LR&referrer=%5Bthe%20profile%20of%20Iretiayo%20Akinola%5D(%2Fprofile%3Fid%3D~Iretiayo_Akinola1)
%\caelan{Should we build on HITL-TAMP, MimicGen, or other formulations?}

We address controlling a robot to perform multi-stage manipulation.
The robot is tasked with manipulating one or more movable objects $o \in O$ in the world to achieve a goal.
The robot observes RGB-D images, which it can process into segmented point clouds for each object ${\cal P} = \{o:P_o \mid o \in O\}$.
Although we assume that we can detect the category of each object, critically, we do not assume available to geometric model of any object ({\it e.g.} mesh).

The state of the world is described by robot configuration $q \in \mathbb{R}^d$ and frame state $S = \{o: \T{o}{w} \mid o \in O\}$, where $\T{f_1}{f_2} \in \SE{3}$ represents a rigid transformation from frame $f_1$ to $f_2$ and $w$ is the world frame.
Let $\R{S}{f_1}{f_2}$ be shorthand for the rigid transformation from frame $f_1$ to $f_2$ in state $S$.
The robot takes actions $a = \T{e}{a}$ that correspond to target end-effector poses, where $e$ is the end-effector frame.
These task-space set points are converted to joint-space commands using Operational-Space Control (OSC)~\cite{khatib1987unified}.

We are interested in re-purposing a set of 
%task and individual skill 
demonstrations for an ensemble of tasks into a manipulation policy that is effective in scenes with new objects and varying initial poses.
To that end, we assume a dataset of demonstrations that is collected by human teleoperation or some other process.
Let a demonstration trajectory $\tau = [\langle S_1, a_1 \rangle, ..., \langle S_h, a_h \rangle]$ be a sequence of state-action pairs $\langle S, a \rangle$.

\subsection{Skill Demonstrations}

In order to deploy demonstrations to new objects and tasks, we need to understand more about the context behind each action: which objects are interacting or are about to interact, and qualitatively how they are interacting.
In this work, we assume that each state-action pair $\langle S, a \rangle$ can be labeled with an interaction type $l$, a source movable object $o$, and target coordinate frame $f$, forming a tuple $\langle l, o, f, S, a \rangle$.
% Where does this come from - manual human annotation
Our technique will be to characterize the motion of $o$ relative to $f$ using NDFs and then adapt it to new circumstances.
Fig.~\ref{fig:ndf_interact} demonstrates a pair of insertion interactions involving pegs and holes that vary in geometry.
Here, the movable object $o$ is the peg and the target frame $f$ is the hole.

\begin{figure}
  \begin{center}
    \includegraphics[width=1\linewidth]{images/NDF_interaction.pdf}
    % \vspace{-5pt}
  \end{center}
  \caption{\textbf{Trajectory Adaptation.} An illustration depicting how an insertion demonstration for a Peg \& Hole combination (left) can be adapted to a new Peg' \& Hole' combination at test time.
  %Illustration of generating a new motion trajectory for test scenario based on the reference demonstration. 
  }
  % \caelan{Hole' frame}}
  \label{fig:ndf_interact}
  \vspace{-12pt}
\end{figure}

%Our objective is to re-purpose these labeled demonstrations into reusable components.
Once provided a labeled demonstration, we can temporally segment and collapse contiguous state-action pairs with the same label into a sequence of trajectories, producing a {\em segmented demonstration} $[\langle l_1, o_1, f_1, \tau_1 \rangle, ..., \langle l_h, o_h, f_h, \tau_h \rangle]$, where each segment represents a {\em skill}.
Still, these demonstrations are currently specialized toward specific 1) object geometries and 2) initial poses.

To generalize them, we transform them using NDFs by extracting the pose of the target frame $f$ relative to the observed object $o$.
Specifically, for each demonstration data point $\langle o, f, S, a \rangle$ and current point cloud $P_o$ for object $o$, we 
% map the action $a$ to its 
compute the NDF feature $z {\gets} F(\R{S}{f}{w} \mid P_o)$ of the pose of frame $f$ relative to observed object $o$.
When applied to a state-action trajectory $\tau$, this results in a {\em feature trajectory} ${\cal Z} = [z_1, ..., z_k]$.
%which can be computed efficiently by using warm starts from the prior state during the NDF optimization.
And when applied to a segmented demonstration, this produces a {\em feature demonstrations}
$d = [\langle l_1, o_1, f_1, {\cal Z}_1 \rangle, ..., \langle l_h, o_h, f_h, {\cal Z}_h \rangle]$.
% Need observation in demonstrations
Thus, we accumulate a {\em skill dataset} of feature demonstrations ${\cal D} = \{d_1, ..., d_n\}$, which can includes demonstrations that span multiple tasks.

\subsection{Peg-in-Hole Example} \label{sec:example}
%\subsection{Interactions / Skills / Action Types }

%In order to plan, we need a model of our labeled interactions.

Continuing the ``Peg-in-Hole" running example in Fig.~\ref{fig:ndf_interact}, we discuss relevant skills and plans.
%To complete the task, the robot must insert the peg object into the hole peg.
It requires two types of interactions: 1) moving the end-effector to grasp an object and 2) inserting a grasped object into another entity.
%Both of these relate to a $\langle l, o, f, z \rangle$ tuple, where $l \in \{\proc{grasp}, \proc{attach}\}$.
These interactions can be formalized by the following planning operators, where $l \in \{\proc{grasp}, \proc{attach}\}$:
%\noindent NDF actions
\begin{enumerate}
    \item $\proc{grasp}(o, e; {\cal Z})$: move to grasp object $o$ with end-effector frame $e$ 
    %using trajectory $\tau$.
    using feature trajectory ${\cal Z}$.
    \item $\proc{insert}(o, f; {\cal Z})$: while grasping object $o$, move to insert $o$ relative to frame $f$ 
    %using trajectory $\tau$.
    using feature trajectory ${\cal Z}$.
\end{enumerate}
% Z instead of \tau
% Feature vectors
A plan that adapts the demonstrations has the following form:
\begin{align*}
    \pi = [&\proc{grasp}(\text{peg}, \text{ee}; {\cal Z}_1), \proc{insert}(\text{peg}, \text{hole}; {\cal Z}_2)].
\end{align*}
%$\widehat{\pi} = [\langle \proc{grasp}, \text{peg}, \text{ee}\rangle, \langle \proc{attach}, \text{peg}, \text{hole}\rangle]$

In between the contact-involved component of these interactions are contact-adverse robot movement.
We can plan motions between the end of the last component and the start of the next one in order to more robustly and efficiently move between segments.
These segments can also be represented by planning operators~\cite{simeon2004manipulation}:
\begin{enumerate}
    \item $\proc{transit}(\tau)$: while not grasping any object, move the robot along trajectory $\tau$.
    \item $\proc{transfer}(o; \tau)$: while grasping object $o$, move the robot along trajectory $\tau$.
\end{enumerate}
A plan that includes motion operators has the following form:
\begin{align*}
    \pi = [&\proc{transit}(\tau_1), \proc{grasp}(\text{peg}, \text{ee}; {\cal Z}_1), \\
    &\proc{transfer}(\text{peg}; \tau_2), \proc{attach}(\text{peg}, \text{hole}; {\cal Z}_2)]
\end{align*}
% Still need to understand that frames are connect to same object
% Category-level scene graph

\section{\Ours}

\begin{figure}[t!]
  \begin{center}
    % left, bottom, right and top
    % \includegraphics[trim={0.5cm 0.6cm 0.8cm 0.1cm}, clip, width=\linewidth]
    \includegraphics[width=\linewidth]
    {images/nod_pipeline.pdf}
  \end{center}
  \caption{\textbf{\Ours System.} 
  %An overview of the \Ours system. 
  Given a goal specification, a task planner plans a sequence of skill types. Then, a skill reasoner searchers for the combination of skill demonstrations that maximizes compatibility. Using NDFs, each selected skill demonstration is adapted to the current scene. Finally, the adapted skills are executed in sequence.
  }
  \label{fig:system}
  \vspace{-10pt}
\end{figure}
We present algorithms for adapting a dataset of skill demonstrations to new problems.
First, we show how a single skill demonstration can be adapted to a new environment using NDFs (Section~\ref{sec:adapt}).
Then, we propose a planning algorithm that's able to combine skill segments from multiple demonstrations to maximize compatibility (Section~\ref{sec:plan}).
Finally, we use motion planning to connect each skill in order to efficiently and robustly generalize to new environments (Section~\ref{sec:motion}). 
%For simplicity, we compute plans offline and execute them open loop.
{The workflow for \Ours is illustrated in Fig.~\ref{fig:system}.}

\subsection{Trajectory Adaptation}\label{sec:adapt}

%\caelan{Describe directly adapting source trajectories (similar to MimicGen)}

\begin{algorithm}[!ht]
  \begin{small} % footnotesize
  \caption{Trajectory adaptation}
  \label{alg:adaptation}
  \begin{algorithmic}[1] % The number tells where the line numbering should start
    \Declare Segmented point clouds ${\cal P}$
    \Declare Initial end-effector pose $\R{S}{e}{w}$
    %\Declare Trajectory sequence ${\cal T}$
    \Declare Demonstration dataset ${\cal D} = \{d_1, ..., d_n\}$
    \Declare NDFs ${\cal F}$
    \Procedure{adapt-traj}{${\cal P}, \R{S}{e}{w}, d; {\cal F}$}
        \State ${\cal S} = \{f: \proc{ndf-estimate}({\cal P}, f) \mid f \in F\} \cup \{e:  
        \R{S}{e}{w}\}$
        \State $G \gets \{\;\}$ \Comment{Object scene graph}
        \For{$\langle l, o, f, {\cal Z} \rangle \in d$}
            \For{$z \in {\cal Z}$}
                \State $T_{z} \gets \proc{ndf-optimize}({\cal F}[o], {\cal P}[o], z)$
                \State $\R{S}{e}{w}, \R{S}{f}{w} \gets {\cal S}[e], {\cal S}[f]$ \Comment{End-effector \& frame}
                \If{$o \in G$} \Comment{Relative to scene graph}
                    \State $\langle f', \R{T}{f'}{w}\rangle \gets G[o]$
                    \State $\R{S}{f'}{w} \gets S[f']$      
                    \State $\T{f}{w} \gets \R{S}{f'}{w} \cdot (\R{T}{f'}{w})^{-1} \cdot T_{z}$
                \Else \Comment{Relative to world frame}
                    \State $\T{f}{w} \gets T_{z}$
                \EndIf
                \State $\R{T}{e}{w} \gets \R{S}{e}{w} \cdot (\R{S}{f}{w})^{-1} \cdot \T{f}{w}$ \Comment{End-effector target}
                \State \Comment{If $f = e$, this reduces to $\R{T}{e}{w} \gets \T{f}{w}$}
                \State \Yield{} $\langle l, o, f, \R{T}{e}{w} \rangle$ \Comment{Yield target to controller}
                \State $S[e] \gets \R{T}{e}{w}$
            \EndFor
            % Condition on interaction type?
            \State $G[o] \gets \langle f, \R{S}{f}{w} \rangle$ \Comment{Set $f$ as the parent of $o$}
        \EndFor
    \EndProcedure
\end{algorithmic}
\end{small} % footnotesize
\end{algorithm}

% Shou adapts trajectories without simulation so it's not actions
% Stacking (more general kinematics)
% Observable vs partially observable
% Offline vs online

Our first algorithm directly adapts a demonstration $d$ to the current task.
%Similar to MimicGen + NDF~\cite{mandlekar2023mimicgen}
Algorithm~\ref{alg:adaptation} displays the trajectory adaptation pseudocode.
It iterates over each labeled feature trajectory in demonstration $d$ and then over each timestep in the trajectories.
For each timestep, it computes the target transformation $T_z$ that corresponds to NDF feature $z$.
Depending on whether object $o$ is attached to another frame $f'$ in the scene graph $G$, it composes the transform into a target world pose $\R{T}{f}{w}$ for manipulation frame $f$.
It converts this into a target end-effector pose $\R{T}{f}{w}$, which will serve as a setpoint for a downstream controller or planner.
After iterating over a labeled trajectory, the scene graph $G$ is updated with the new state of the manipulated object $o$.
This also models the point cloud $P_o$ for object $o$ as being attached to (and thus moving with) frame $f$.

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=1.\linewidth]{images/skill_reasoning.pdf}
  \end{center}
  \caption{\textbf{Skill Planning and Trajectory Adaptation.} 
  On this representative mug insertion task, \Ours first selects a sequence of compatible skills by checking their NOD feature compatibility (Sec.~\ref{ssec:planning}). The trajectory is then adapted using Algo.~\ref{alg:adaptation} for the current scene. Finally, a motion planner generates transitory motion between the adapted skills (Sec.~\ref{sec:motion}).%  If a transition is deemed infeasible (e.g., collision), then a new demo is selected to replace the %the NOD feature from the start state and end state of the reference demo to infer the test object poses. It then transforms the object point cloud with the inferred pose to propagate the future point cloud scene states, which is used by the motion planner for collision checking. Once deemed feasible by the motion planner, 
  }
  % \vspace{-10pt}
  \label{fig:skill_reasoning}
\end{figure}


%\subsection{Task and Motion Planning}
\subsection{Skill Planning}\label{sec:plan}
\label{ssec:planning}
%Adapting an entire demonstration trajectory may be unsuitable in many cases -- for example, if the {\em plan skeleton}, or the sequence of skills changes from the reference demonstration. This motivates the capability to use segments of multiple demonstrations together. As an example, it might be possible to adapt the picking part of a pick-and-place mug demonstration to interact with a new object (a bowl, for instance), or re-use part of an existing demonstration to achieve a new goal.

% It can be limiting to be only able to reuse whole demonstrations.
% First, it is inflexible in problems where the, {\em plan skeleton}, or the sequence of skills changes.
% Second, segments of multiple demonstrations in conjunction might better address a new problem. For example, we may just transfer the picking part of the pick-and-place trajectory that work with a mug to interact with a new object, e.g., a bowl.

% https://github.com/touristCheng/robomimic-hitl/blob/c68e89334c468f3164ab04d63bc586260f7c015b/robomimic/scripts/traj_optim_full_task_%2Bmp.py#L902
\begin{algorithm}[!ht]
  \begin{small} % footnotesize
  \caption{\Ours planner}
  \label{alg:planner}
  \begin{algorithmic}[1] % The number tells where the line numbering should start
    \Declare Plan skeleton $\widehat{\pi} = [\langle l_1, o_1, f_1 \rangle, ..., \langle l_h, o_h, o_h \rangle]$ % Capitalize
    \Procedure{plan-ndf-skills}{${\cal P}, \widehat{\pi}; {\cal D}, {\cal F}$}
        \State $D = [\;]$ \Comment{List of demos per skill}
        \For{$\langle l_i, o_i, f_i \rangle \in \widehat{\pi}$}
            \State $D \gets D + [\{\langle l, o, f, {\cal Z} \rangle \mid d \in {\cal D}, \langle l, o, f, {\cal Z} \rangle \in d.\; \newline l {=} l_i \wedge o {=} o_i \wedge f {=} f_i\}]$
        \EndFor
        \State $\pi_* \gets \None$; $c_* \gets \infty$
        %\caelan{Sort instead of min?}
        \For{$\pi \in \proc{product}(D_\pi )$} \Comment{All combinations} % Cartesian product, DFS
            \State $c_\pi \gets 0$ \Comment{Feature cost}
            \For{$i \in [1, ..., |\pi|{-}1]$}
                % \State $\langle o_i, f_i \rangle, \langle o_{i+1}, f_{i+1} \rangle \gets \pi[i], \pi[i+1]$
                % \State ${\cal Z}_i, {\cal Z}_{i+1} \gets \pi[i], \pi[i{+}1]$
                \State $\langle l_i, o_i, f_i, {\cal Z}_i \rangle \gets \pi[i]$
                \State $\langle l_{i+1}, o_{i+1}, f_{i+1}, {\cal Z}_{i+1} \rangle \gets \pi[i{+}1]$
                \If{$o_i = o_{i+1}$} \Comment{Actions with same object}
                    \State $F \gets {\cal F}[o]$; $P \gets {\cal P}[o]$
                    \State $T_i \gets \proc{ndf-optimize}(F, P, {\cal Z}_i[-1])$
                    \State $T_{i+1} \gets \proc{ndf-optimize}(F, P, {\cal Z}_{i+1}[0])$
                    \State $z_i, z_{i + 1} \gets F(T_i \mid P), F(T_{i+1} \mid P)$
                    \State $c_\pi \gets c_\pi + ||z_{i + 1} - z_i||$ % _2
                    %\todo{Shuo: since you haven't shared the equation yet, this is my best guess}
                \EndIf
            \EndFor
            %\State \caelan{Goal constraints?}
            \If{$c_\pi < c_*$} \Comment{Update best plan}
                \State $\pi_* \gets \pi$; $c_* \gets c_\pi$
            \EndIf
        \EndFor
        %\caelan{Filter trajectories?}
        \State \Return $\pi_*$
    \EndProcedure
\end{algorithmic}
\end{small} % footnotesize
\end{algorithm}
% https://github.com/touristCheng/robomimic-hitl/blob/htamp_dataset_mp/robomimic/scripts/traj_optim_full_task_%2Bmp.py#L1263
Given a set of skill demonstrations, the goal of the skill planner is to select a sequence of skills that can be chained together to reach a task goal.
Algorithm~\ref{alg:planner} displays the pseudocode for the \Ours planner.
It takes in a plan skeleton $\widehat{\pi}$ that defines a sequence of skill types to consider.
% Future work
It first compiles a list of skill demonstrations in dataset ${\cal D}$ relevant to $\pi$.
Then, it iterates through all possible plans using these skills.
Each candidate $\pi$ is scored based on the compatibility of subsequent actions using NDF features, the score $c$ is computed as
$c = \sum_{i=1}^{|\pi|{-}1} ||z_{i + 1} - z_i||$
, where for specific $i$, the NDF feature $z_i$ and $z_{i+1}$ are extracted as:
\begin{equation*}
z_i, z_{i + 1} \gets F(T_i \mid P), F(T_{i+1} \mid P)
\end{equation*}

Here $T_i$ and $T_{i+1}$ are the query pose determined at the last time step and first time step of the trajectories from skill $i$ and skill $i+1$ respectively, and $P$ is the point cloud of the target object for skill $i$ and skill $i+1$ captured during demonstration.

% \caelan{Shuo: add a standalone equation for the cost here}
After we obtain all scores for all skill combinations, the plan with the lowest plan-wide NDF feature distance is returned. For simplicity, we present this as a Cartesian product over relevant skills, but this can be done more efficiently by performing a Uniform Cost Search in plan space, where the NDF feature distance serves as a the cost function. Fig.~\ref{fig:feat_match} visualizes the feature matching process for a mug placing example.
It demonstrates that grasping the mug on its rim is compatible with placing the mug upright in a bin and grasping it on its handle is compatible with inserting it into a cabinet.

% plan-space Depth-First Search (DFS)
% Precondition?

\begin{figure}[t!]
  \begin{center}
    \includegraphics[width=1.\linewidth]{images/feat_match.png}
  \end{center}
  % \caption{\textbf{Feature Matching.} The feature matching distance for different skill combinations when placing a mug. In this example, for characterizing the relationship between the mug and the end-effector, we use the NOD feature extracted from the mug point cloud and the end-effector pose in the mug frame, for representing the relationship between mug and cabinet, we use the NOD feature extracted from the mug point cloud and the cabinet pose.}
  \caption{\textbf{Feature Matching.} The NOD feature matching distance for different skill combinations when placing a mug in different ways. The NOD feature extracted from the mug point cloud and the end-effector pose is used to characterize the relationship between the mug and the end-effector, and the NOD feature extracted from the mug point cloud and the container (e.g., cabinet) pose is used to represent the relationship between the mug and the container. Grasping the mug on its rim is compatible with placing the mug upright in a bin and grasping the mug on its handle is compatible with inserting it into a cabinet. This allows \Ours to adapt different demonstration pieces to accomplish different goals.}
  \label{fig:feat_match}
  \vspace{-10pt}
\end{figure}


%\subsection{Motion Planning}
%\subsection{Motion Refinement}
\subsection{Transit \& Transfer Motion}
\label{sec:motion}

Adapting demonstrated skills is particularly effective at generating behavior that involves contact.
However, demonstrations typically contain long segments without contact (outside of holding an object). Because these components do not modify the world, it is often not productive to replicate them.
Thus, we temporally trim skill demonstrations to focus on the data points that involve contact. In our implementation, we simply select the 50 steps before contact.
% \caelan{Shuo: give specific criteria}

After trimming, and in often before trimming, two adjacent skills might be far away in task space.
While linear interpolation is an option, this is not generally safe because the straight-line path may cause the robot to unexpectedly collide.
To address this, we use motion planning to optimize for safe and efficient motion that reaches the start of next the skill.
Motion planning generally requires some characterization of the collision volume of the obstacles to avoid.
Because we do not assume access to object models, we use the segmented point clouds ${\cal P}$ as the collision representation, where each point in the cloud is a sphere with radius $r > 0$.

\begin{algorithm}[!ht]
  \begin{small} % footnotesize
  \caption{\Ours policy}
  \label{alg:policy}
  \begin{algorithmic}[1] % The number tells where the line numbering should start
    \Procedure{\Ours-policy}{${\cal P}, \pi; {\cal D}, {\cal F}$}
        \State $\pi \gets \proc{plan-ndf-skills}({\cal P}, \pi; {\cal D}, {\cal F})$
        \If{$\pi = \None$}
            \State \Return \False \Comment{Skill planning failed}
        \EndIf
        \State $a \gets \None$ \Comment{Current action}
        \State $\R{S}{e}{w} \gets \proc{forward-kin}(q)$
        \For{$\langle o, f, \R{T}{e}{w} \rangle \in \proc{adapt-traj}({\cal P}, \R{S}{e}{w}, \pi; {\cal F}$)}
            \If{$\langle o, f \rangle \neq a$} \Comment{Action changed}
                \State $a \gets \langle o, f \rangle$ \Comment{Update current action}
                \State $q \gets \proc{observe-conf}()$
                \State $\tau \gets \proc{plan-motion}({\cal P}, q, \R{T}{e}{w})$
                \If{$\tau = \None$}
                    \State \Return \False \Comment{Motion planning failed}
                \EndIf
                \State $\proc{execute-traj}(\tau)$
            \EndIf
            \State $q \gets \proc{observe-conf}()$
            \State $\proc{execute-osc}(q, \R{T}{e}{w})$ \Comment{Operational Space}
        \EndFor
        %\State \proc{adapt-trajectory}($S_0, \pi$)
        \State \Return \True \Comment{Policy succeeded}
    \EndProcedure
\end{algorithmic}
\end{small} % footnotesize
\end{algorithm}
%\caelan{What exactly are the goal constraints in our domains?}
%\caelan{Sum of task score and comp score}
% Observation where the observation could just be the state
% Label $l = \langle x, f, f' \rangle$
% Vector notation for a plan
% Different labels per pair for frames
% Online vs offline
% Learned action constraints
% Plan-space planner

Algorithm~\ref{alg:policy} displays the pseudocode for the full \Ours policy with motion planning.
It is shown with online motion planning and execution, but full plans can also be computed offline.
The policy first computes a skill plan $\pi$ and then adapts each labeled trajectory in sequence.
Between adapted trajectories, it uses \proc{plan-motion} to plan a trajectory from the current robot configuration $q$ to a configuration that reaches the first end-effector pose $\R{T}{e}{w}$.
Specifically, it samples goal configurations $q'$ using inverse kinematics and then invokes a sampling-based motion planner between $q$ and $q'$.
% Holding
Once the end-effector arrives at $\R{T}{e}{w}$, for each pose yielded by the skill, the policy uses an Operational Space Controller (OSC)~\cite{khatib1987unified} to track the target poses. 

A detailed example of how the system works for placing the mug into the cabinet is presented in Fig.~\ref{fig:skill_reasoning}. The skill planning process first identifies the reference trajectories for the pick and place skills by matching constraint features (see Fig.~\ref{fig:feat_match} for an example).
These trajectories are adapted to the test scene using NDFs.
Then, a motion planner generates transitory motion between these trajectories. 
% Once the motion transition among every connections between the consecutive skills are determined, we transfer the trajectories to the test scene through trajectory adaptation. 
Altogether, the planning time is typically 1-2 minutes, where the NDF optimization is most of the runtime.
These algorithms can be run online while the robot is executing to minimize the overall task time.


==> text/MethodRetired.tex <==
\section{Retired}
%\section{\Ours}

\caelan{Will need to merge with my additions}

We aim to design a framework that enables robots to solve and generalize across long-horizon tasks, with just a handful of human demonstrations on individual short-horizon tasks. The main challenges are: 1) daily objects have diverse shapes and the scene involves diverse object pose combinations, but for in-the-wild situations, it is usually hard to obtain object models; 2) daily tasks are usually long-horizon, which needs reasoning and coordination of different individual actions to complete. To tackle these challenges, we propose \Ours, a framework that \todo{summarize}. Our framework includes: 1) a skill reasoning module that identifies and sequential the suitable demonstrated trajectories in a correct order based on the final goal representation; 2) a trajectory adaptation component that transfers the reference trajectory based on the test object shape and pose, which enables generalization over diverse object geometry and pose configurations. We will describe each module in details in the following sections.

\todo{Introduce overall system, refer to pipeline figure;}

Our \Ours system is compatible with a wide range of off-the-shelf task and motion planning frameworks, as long as these frameworks offer a comparable interface for handling perceptual elements and planning outputs. 
% In this work, we utilize PDDLStream~\cite{garrett2020pddlstream} to instantiate our system. 
% \todo{Introduce PDDLStream}

\subsection{NDF for Trajectory Generation}

\todo{Optimize query trajectory in the NDF object frame}

\todo{Treat reference object as with canonical pose and estimate NDF object pose, which is used to provide a good initialization for optimization}

\subsection{Operators with Neural Constraints}

\todo{Introduce operator definition, e.g., precondition/effects as constraints represented with NDF features}

\todo{Introduce operator grounding and skill reasoning for demo selection, maybe use pseudo algorithm to show the DFS search process}

\subsection{Integrated \Ours}
\todo{Skill instance representation, record eef trajectory and relative pose between contact and moving object, transferring relative pose (constraints) to test object. Then use the obtained constraints to construct the kinematics chain, e.g., $T_{a2b} = T_{q2b} \cdot T_{q2a}^{-1}$, and infer the transform between the query and eef.}

\todo{Use NDF constraints to derive ending eef pose of previous skill and starting eef pose for subsequent skill, use motion planning for skill transition. Use derived object poses to transform object point clouds to forecast future scene states, which is used for collision checking during motion planning.}

\todo{Explain deferred NDF trajectory optimization to improve efficiency, refer to figure. After obtaining the query trajectory in the world frame, we can derive the eef trajectory in world, chain up all eef trajectory segments for execution.} 

\subsection{Experiment Plan}

\begin{enumerate}
    \item Method comparison on new shapes (maybe easy and hard, to highlight trajectory adaptation is needed compared to NDF) (MugPicking: just pick up mug, different shapes, same pose)
    \item Method comparison on new object poses - wide generalization (maybe highlights value of motion planner component too? SameMugPickingRandomPose, Low and High Variance Dists) 
    \item Method works on both new shapes and new poses for single stage tasks (MugPickingRandomPose)
    \item Method can be applied to multi-stage manipulation with multiple objects (number of subtasks, number of objects and receptacles, TableClearSame: place two mug in bins, ToolHang)
    \item Method can appropriately use different strategies from reference demos to achieve goals (both single-stage and multi-stage, TableClearHard: place one mug in bin, one in cabinet)
    \item Method works on substantial variations (pose, objects) across long-horizon tasks (TableClearHard)
    \item Method can generalize to several different long-horizon goal variations without the need to recollect any human data (this includes re-purposing skills from human data in different ways in the same episode, TableClearHard)
    \item Method can be applied to contact-rich manipulation and diverse skills (insertion, hanging, not just pick and place) as well (unlike NDF) - ToolHang, MugInsertion)
    \item \caelan{Multi-object interactions (e.g. Tool Hang, stacking, packing)}
    \item \caelan{Reason about geometric constraints limiting demonstrations (e.g. pick/place collisions)}
\end{enumerate}

todo rankings: 
\begin{itemize}
    \item 6) TableClearHard (finished, in table 1)
    \item 4) TableClearSame: (only 1 pick strategy, 1 place strategy)
    \item ToolHang
    \item MugPickingVairants
    \item 8) MugInsertion (only 1 mug, 1 cabinet, reduce tol)
\end{itemize}

==> text/Method_revised.tex <==
%\section{Background and Prerequisites}
\section{Problem Overview and Formalization}
%\section{Few-shot Manipulation for Unknown Objects}
\label{sec:method}
\subsection{Problem Overview}
\revise{The central question we aim to answer is: \emph{given a set of demonstration trajectories, can we adapt and recompose them to solve new tasks with new objects and scenes?} Our solution adopts the TAMP framework, where a high-level planner orchestrates a set of short-horizon motion generators (skills) to produce coherent long-horizon plans. The framework allows us to divide the problem into three technical sub-problems. (1) How to represent demonstration trajectory snippets as TAMP skills? In particular, how should we represent their precondition and effect constraints? (2) How to adapt skills instantiated with recorded trajectories to new scenes and objects? (3) Given a new task goal, how to chain these skills together to generate a trajectory plan?}

\revise{Our insight is that NOD features will enable us to adapt both motion trajectories and skill constraints to new scene layouts and object shapes.  Our goal is to develop a cohesive TAMP framework that addresses these sub-problems by building its core components on NOD representations. Below, we will introduce the problem setting (Section~\ref{sec:problem}), review a specific instance of NOD representation that we adopt~\cite{simeonovdu2021ndf} (Section~\ref{sec:ndf}), present our demonstration and skill representations (Section~\ref{sec:skill_repr}), and give an illustrative example (Section~\ref{sec:example}).}

% introducing the problem formulation, the concept of our framework, the input and output of our system, the requirements and conditions for implementing the system, and the scenarios and advantages of the framework.

%\todo{Problem formulation, concept, requirements for inputs/observations, outputs, advantages (handling novel unknown objects, acquisition of new skills with few demonstrations, easy to support continuous skill integration)}

% \revise{Our framework leverages NDFs~\cite{sundermeyer2021contact}, a type of Neural Object Descriptor, for both few-shot skill learning and multi-step skill reasoning.} First, we review background on NDF for category-consistent frame estimation (Section~\ref{sec:ndf}).
% Then, we describe our problem setting (Section~\ref{sec:problem}).
% \ajay{Need more of an overview here. For example. Task Demonstrations in Section C comes out of nowhere. The ending text in section B is very good as a guide for the method, and should be moved here as part of the overview.}



\subsection{Problem Setting} \label{sec:problem}

% MimicGen: A Data Generation System for Scalable Robot Learning using Human Demonstrations
% https://openreview.net/forum?id=dk-2R1f_LR&referrer=%5Bthe%20profile%20of%20Iretiayo%20Akinola%5D(%2Fprofile%3Fid%3D~Iretiayo_Akinola1)
%\caelan{Should we build on HITL-TAMP, MimicGen, or other formulations?}

We seek to control a robot to perform multi-stage manipulation. 
The robot is tasked with manipulating one or more movable objects $o \in O$ in the world to achieve a goal.
The robot observes RGB-D images, which it can process into segmented point clouds for each object ${\cal P} = \{o:P_o \mid o \in O\}$.
Although we assume that we can detect the category of each object, critically, we do not assume access to geometric models of any object ({\it e.g.} mesh).

\revise{The state of the world is described by robot configuration $q \in \mathbb{R}^d$ and scene graph $G = \{o: \langle P_o, \T{{o}}{{w}} \rangle \mid o \in O\}$, where $\T{\mathrm{a}}{\mathrm{b}} \in \SE{3}$ represents a rigid transformation from frame $\mathrm{a}$ to $\mathrm{b}$ and ${w}$ is the world frame.
% Let $\R{S}{f_1}{f_2}$ be shorthand for the rigid transformation from frame $f_1$ to $f_2$ in state $S$.
The robot takes actions $a = \T{{e}}{{w}}$ that correspond to target end-effector poses, where ${e}$ is the end-effector frame, and $\T{{o}}{{w}}$ is the recovered pseudo object pose using above mentioned method.}
\ajay{Consider adding an equation ref at end of section A, so we can refer to it here.}
These task-space set points are converted to joint-space commands using Operational-Space Control (OSC)~\cite{khatib1987unified}. \ajay{Consider mentioning control rate of actions here, so it's clear that the robot tries to track waypoints at a certain rate.}

We are interested in re-purposing a set of 
task and individual skill 
demonstrations for an ensemble of tasks into a manipulation policy that is effective in scenes with new objects and varying initial poses.
Thus, we assume a dataset of demonstrations that is collected by human teleoperation or some other process.
% Let a demonstration trajectory $[\langle S_1, a_1 \rangle, ..., \langle S_h, a_h \rangle]$ be a sequence of state-action pairs $\langle S, a \rangle$.


\subsection{Neural Descriptor Fields (NDF)} \label{sec:ndf}
%\caelan{Appears to be a subset of "Problem Formulation"}

NDF~\cite{simeonovdu2021ndf} were first proposed for category-invariant modeling of object rigid transformations. 
\ajay{Some of the terminology is out of order here -- e.g. $F(T|P)$ without describing what T is (which comes later). Also, does X not appear in the NDF? e.g. $F(T|P, X)$}
\revise{A NDF pose encoder $\posendf(T \mid P)$ takes in an object shape that is represented as a point cloud $P \in \mathbb{R}^{N\times3}$ and a set of query positions $\{R \cdot x_i+t \mid x_i \in X\}$.
Let $T = [R \mid t] \in \SE{3}$ be a rigid transformation and $X \in \mathbb{R}^{M\times3}$ be a vector of query points. We define $\pointndf$ as a learned model that maps a single query coordinate to a feature vector, and $\posendf$ as an operation that maps a query pose $T$ to an extended feature descriptor $z$ by concatenating all the features of a set of query coordinates parameterized by the query pose}:

\begin{equation*}
z \gets \posendf(T \mid P) \equiv \bigoplus_{x_i \in X} \pointndf(R \cdot x_i+t \mid P).
\label{eq:pose_enc}
\end{equation*}

A key advantage of NDF features is that they are only related to the queries in the object's local frame, therefore a rigid transformation $R \in \SE{3}$ applied to both the shape and the query pose has no affect on the feature:
%would affect the extracted feature, which allows us to generalize the extracted pose $R \cdot T$ with arbitrary configuration $R$ of the new shape:
\begin{equation*}
\posendf(R \cdot T \mid R \cdot P) = \posendf(T \mid P).
\label{eq:pose_enc}
\end{equation*}

NDFs are typically used to solve an inverse problem: recover a transformation $T$ that corresponds to a query feature $z$.
This can be framed as the following optimization problem and solved by 1) randomly initializing the transform, 2) backpropgating to compute the error gradient, and 3) iteratively moving along the gradient to minimize the error:
\begin{equation*}
% \proc{ndf-optimize}(P, \posedescriptor) \equiv \underset{T}{\text{argmin}} ||\posedescriptor -  \posendf(T \mid P)||_1
\proc{ndf-optimize}(F, P, z) \equiv \underset{T}{\text{argmin}} ||z -  \posendf(T \mid P)||. % _1
\end{equation*}

\danfei{Why do we need this paragraph here?}\revise{Please be aware that NDFs can also be used to estimate novel object $\overline{P}$'s pose $\overline{T}$ w.r.t. a given reference object $P$ with pose $T$. To do so, we can simply define the rotation of $T$ as identity, and define translation as the mean of $P$:}
\revise{
\begin{equation*}
\overline{T} = \underset{T_{i}}{\text{argmin}} ||\posendf(T \mid P) -  \posendf(T_{i} \mid \overline{P})||.
\end{equation*}
}

%Given a reference pose $T$ and a reference object $P$, we can first obtain the corresponding feature $z$. 
%To obtain the new pose $T'$ that maps points from the base frame to the geometric equivalent positions in the new shape's frame, we can randomly initialize the new pose and back-propagate the gradient to it: 

% \begin{equation*}
% T' = \underset{T'}{\text{argmin}} ||z - \posendf(T' \mid P')||.
% \label{eq:pose_enc}
% \end{equation*}
%Let the following solve for a transformation $T$ that matches NDF feature $z$:

\subsection{Skills and Constraints}
\danfei{We need a section to clearly explain what we mean by skills and their constraints with minimum notations, Fig 13 will help here. We should explain it to the point where it is clear where NDF can be used to make the skill and their constraints more general. I'd just delete the entire next subsection and explain how we make it adaptable as ``our method''.}

\subsection{Task Demonstrations and Skill Representations}
\label{sec:skill_repr}
In order to deploy demonstrations to new objects and tasks, we need to understand more about the context behind each action: which objects are interacting or are about to interact, and qualitatively how they are interacting. Our technique will be to characterize the relative motion of two objects (represented by the relative transform between a query frame $q$ of one object to another object) using NDFs and then adapt it to new circumstances.
% \revise{In this work, we assume that each state-action pair $\langle S, a \rangle$ can be labeled with a skill name $l$ (e.g., \proc{pick}), a source object $o_{s}$ which represented as $P_{o_s}$ that has a corresponding NDF model $f_{o_s}$, and a query pose $\T{{q_m}}{{o_m}}$ that defined in the target object $o_{m}$'s local frame, forming a tuple $\langle l, o_s, o_m, \T{{q_m}}{{o_m}}, S, a \rangle$.}


\revise{In this work, we propose to represent each skill as a tuple: $\langle l, o_{src}, o_{tgt}, \T{{q_{tgt}}}{{o_{tgt}}}, P_{o_{src}}, P_{o_{tgt}}, \tau,  C_{req}, C_{del}, C_{add}\rangle$, where $l=\langle\textit{name}, \textit{mode}\rangle$ represents the skill name (e.g., \proc{pick}, \proc{insert}) and how the kinematics structure will change ($\textit{mode} \in \{\texttt{attach}, \texttt{detach}\}$), $o_{src}$ and $o_{tgt}$ represent the source object and target object respectively \ajay{are these just object labels? be more explicit here (e.g. be clear they are not poses)}, and we have NDFs ${\cal F}$ for all source object categories \ajay{Why don't we add that into the skill definition? Or maybe mention this assumption in a separate sentence -- it's a little weird right now}. Let $P_{o_{src}}$ and $P_{o_{tgt}}$ represent the point cloud of object $o_{src}$ and $o_{tgt}$, $\T{{q_{tgt}}}{{o_t}}$ denotes a query frame $q_{tgt}$'pose defined in object $o_{tgt}$'s local frame, and $\tau$ represents a sequence of end-effector poses that complete the skill motion. We use $C_{req}$ to denote the set of required constraints of executing the skill, each constraint is a relative transform between two entities, as some skills need (e.g., a \proc{Insert} may require the robot to hold the tool object in a specific way). We use $C_{del}$ and $C_{add}$ to represent the deleted constraints and additive constraints, respectively; for example, after \proc{Insert}, the holding object will detach from the robot hand and be attached to the receptacle, therefore, the constraint transform between the gripper and the holding object is removed, and a new constraint transform between the holding object and the receptacle will be introduced. In this way, we take into account the object geometries and spatial relationships while considering the skill executability.} 

\ajay{There is a lot of new detailed information and notation mentioned above, especially concerning constraints. Maybe we should have an explicit section on notation somewhere? Also, is there something we can cite from TAMP literature about adding and deleting constraints?}

\revise{Here we explain the skill modes and how they influence the relative motion between the source object and target object:
\begin{itemize}
    \item \texttt{attach}: in this case, the robot is trying to grasp a tool object, thus object $o_{tgt}$ is the robot gripper, and object $o_{src}$ is the tool object, $\T{q_{tgt}}{o_{tgt}}$ is defined as identity matrix thus the query frame pose at time step $t$ in the world space $\T{q_{tgt}}{w}^{(t)}$ is the end-effector pose $\T{e}{w}^{(t)}$ recorded in $\tau$;
    \item \texttt{detach}: in this case, the robot is trying to attach the holding object to a receptacle, therefore, object $o_{tgt}$ is the holding object and ${o_{src}}$ is the receptacle object. The query frame pose in the world space at any time step $t$ can be recovered by: $\T{q_{tgt}}{w}^{(t)} = \T{e}{w}^{(t)} \cdot \T{o_{tgt}}{e} \cdot \T{q_{tgt}}{o_{tgt}}$, where $\T{e}{w}^{(t)}$ is the end-effector pose at time step $t$ recorded in $\tau$, and $\T{o_{tgt}}{e}$ is the grasp pose represented in the required constraints $C_{req}$.
\end{itemize}}

\ajay{Since we only have two modes, do we need to acknowledge any limitations of the framework on how general it is?}

% Where does this come from - manual human annotation
% Our technique will be to characterize the relative motion of  $o_m$ relative to $o_s$ using NDFs and then adapt it to new circumstances.
% Fig.~\ref{fig:ndf_interact} demonstrates a pair of insertion interactions involving pegs and holes that vary in geometry. Here, the source object $o_s$ is the peg and the target query frame $\T{q_m}{o_m}$ is defined at the contact region of the hole.

\begin{figure}
  \begin{center}
    \includegraphics[width=1\linewidth]{images/NDF_interaction.pdf}
    % \vspace{-5pt}
  \end{center}
  \caption{\textbf{Trajectory Adaptation.} An illustration depicting how an insertion demonstration for a Peg \& Hole combination (left) can be adapted to a new Peg' \& Hole' combination at test time.
  \revise{better to overlay the skill representation and notations together with reference and test objects to show the concept. maybe merge with figure 13.}
  %Illustration of generating a new motion trajectory for test scenario based on the reference demonstration. 
  }
  % \caelan{Hole' frame}}
  \label{fig:ndf_interact}
  \vspace{-12pt}
\end{figure}

%Our objective is to re-purpose these labeled demonstrations into reusable components.
% Once provided a labeled demonstration, we can temporally segment and collapse contiguous state-action pairs with the same label into a sequence of trajectories, producing a {\em segmented demonstration} $[\langle l_1, o_{s_1}, o_{m_1}, P_{o_{s_1}}, \T{{q_{m_1}}}{{o_{m_1}}}, \tau_1 \rangle, ..., \langle l_h, o_{s_h}, o_{m_h}, \T{{q_{m_h}}}{{o_{m_h}}}, \tau_h \rangle]$, where each segment represents a {\em skill} and $\tau$ is a sequence of end-effector poses. Still, these demonstrations are currently specialized toward specific 1) object geometries and 2) initial poses.

\revise{To generalize a recorded motion to new tasks, at each time step, we want to adapt the relative transforms between the query frame $q_{tgt}$ of target object $o_{tgt}$ and the source object $o_{src}$ to new objects in test scenes using NDFs ${\cal F}$. To facilitate deployment, we compute the NDF feature $z {\gets} F(\T{q_{tgt}}{w} \mid P_{o_{src}})$ of the query frame $q_{tgt}$ relative to observed object $o_{src}$. When applied to a sequence of query poses induced by trajectory $\tau$, this results in a {\em feature trajectory} ${\cal Z_{\tau}} = [z_1, ..., z_{|\tau|}]$. To make the query frame pose be generalizable to query object shape in test scenarios, we compute the NDF feature $z_{q} {\gets} F(\T{q_{tgt}}{w} \mid P_{o_{tgt}})$. We also compute the NDF feature for all constraint transforms, which results in ${\cal Z}_{req}$, ${\cal Z}_{del}$, and ${\cal Z}_{add}$. Therefore, for each single skill, we have feature demo $d = \langle l, o_{src}, o_{tgt}, z_{q}, \cal{Z_{\tau}}, {Z}_\textsubscript{req}, {Z}_\textsubscript{del}, {Z}_\textsubscript{add}\rangle$. And when applied to all recorded skills, this produces a skill dataset of {\em feature demos} ${\cal D} = \{d_1, ..., d_n\}$, which can includes demonstrations that span multiple tasks.}

\revise{Although during data collection stage we record the initial object point clouds as well as the entire end-effector trajectory for the full task, such skill representations can be easily extracted from a task demonstration by annotating the start time step and end time step for each skill, this process can also be automated via detecting the contact between gripper and objects.}

\subsection{Peg-in-Hole Example}\revise{TBD: do we need to switch this example and fig. 2 to mug insertion? also, merge fig2 with fig13 to show skill repr would make the adaptation process more clear} \label{sec:example}
%\subsection{Interactions / Skills / Action Types }

\ajay{Would be useful to have this example use the new terminology introduced in the last section}

%In order to plan, we need a model of our labeled interactions.

Continuing the ``Peg-in-Hole" running example in Fig.~\ref{fig:ndf_interact}, we discuss relevant skills and plans.
%To complete the task, the robot must insert the peg object into the hole peg.
It requires two types of interactions: 1) moving the end-effector to grasp an object and 2) inserting a grasped object into another entity.
%Both of these relate to a $\langle l, o, f, z \rangle$ tuple, where $l \in \{\proc{grasp}, \proc{attach}\}$.
These interactions can be formalized by the following planning operators, where $l \in \{\proc{grasp}, \proc{attach}\}$:
%\noindent NDF actions
\begin{enumerate}
    \item $\proc{grasp}(o, e; {\cal Z})$: move to grasp object $o$ with end-effector frame $e$ 
    %using trajectory $\tau$.
    using feature trajectory ${\cal Z}$.
    \item $\proc{insert}(o, f; {\cal Z})$: while grasping object $o$, move to insert $o$ relative to frame $f$ 
    %using trajectory $\tau$.
    using feature trajectory ${\cal Z}$.
\end{enumerate}
% Z instead of \tau
% Feature vectors
A plan that adapts the demonstrations has the following form:
\begin{align*}
    \pi = [&\proc{grasp}(\text{peg}, \text{ee}; {\cal Z}_1), \proc{insert}(\text{peg}, \text{hole}; {\cal Z}_2)].
\end{align*}
%$\widehat{\pi} = [\langle \proc{grasp}, \text{peg}, \text{ee}\rangle, \langle \proc{attach}, \text{peg}, \text{hole}\rangle]$

In between the contact-involved component of these interactions are contact-adverse robot movement.
We can plan motions between the end of the last component and the start of the next one in order to more robustly and efficiently move between segments.
These segments can also be represented by planning operators~\cite{simeon2004manipulation}:
\begin{enumerate}
    \item $\proc{transit}(\tau)$: while not grasping any object, move the robot along trajectory $\tau$.
    \item $\proc{transfer}(o; \tau)$: while grasping object $o$, move the robot along trajectory $\tau$.
\end{enumerate}
A plan that includes motion operators has the following form:
\begin{align*}
    \pi = [&\proc{transit}(\tau_1), \proc{grasp}(\text{peg}, \text{ee}; {\cal Z}_1), \\
    &\proc{transfer}(\text{peg}; \tau_2), \proc{attach}(\text{peg}, \text{hole}; {\cal Z}_2)]
\end{align*}
% Still need to understand that frames are connect to same object
% Category-level scene graph

\section{\Ours}

\begin{figure}[t!]
  \begin{center}
    % left, bottom, right and top
    % \includegraphics[trim={0.5cm 0.6cm 0.8cm 0.1cm}, clip, width=\linewidth]
    \includegraphics[width=\linewidth]
    {images/nod_pipeline.pdf}
  \end{center}
  \caption{\textbf{\Ours System.} 
  %An overview of the \Ours system. 
  Given a goal specification, a task planner plans a sequence of skill types. Then, a skill reasoner searchers for the combination of skill demonstrations that maximizes compatibility. Using NDFs, each selected skill demonstration is adapted to the current scene. Finally, the adapted skills are executed in sequence.
  }
  \label{fig:system}
  \vspace{-10pt}
\end{figure}
We present algorithms for adapting a dataset of skill demonstrations to new problems.
First, we show how a single skill demonstration can be adapted to a new environment using NDFs (Section~\ref{sec:adapt}).
Then, we propose a planning algorithm that's able to combine skill segments from multiple demonstrations to maximize compatibility (Section~\ref{sec:plan}).
Finally, we use motion planning to connect each skill in order to efficiently and robustly generalize to new environments (Section~\ref{sec:motion}). 
%For simplicity, we compute plans offline and execute them open loop.
{The workflow for \Ours is illustrated in Fig.~\ref{fig:system}.}

\subsection{Trajectory Adaptation}\label{sec:adapt}

%\caelan{Describe directly adapting source trajectories (similar to MimicGen)}

\begin{algorithm}[!ht]
  \begin{small} % footnotesize
  \caption{Trajectory adaptation}
  \label{alg:adaptation}
  \begin{algorithmic}[1] % The number tells where the line numbering should start
    % \Declare Segmented point clouds $\overline{{\cal P}}$
    \Declare Source object in test scene ${o_{src}}$
    \Declare Target object in test scene ${o_{tgt}}$
    \Declare Robot's end-effector $e$
    \Declare Global scene graph $G$
    \Declare Global accumulated constraints $C_{acc}$
    \Declare Demonstration dataset ${\cal D} = \{d_1, ..., d_n\}$
    \Declare NDFs ${\cal F}$
    \Procedure{adapt-traj}{${o_{src}}, {o_{tgt}}, d, {\cal F}$}
        \State $z_{q}, \cal{Z_{\tau}}$ $\gets$ $d$
        \State $P_{o_{src}}$, $\T{{o_{src}}}{w}$ $\gets G[{o_{src}}]$
         \State $P_{o_{tgt}}$, $\T{{o_{tgt}}}{w}$ $\gets G[{o_{tgt}}]$
        \State ${\T{q_{tgt}}{o_{tgt}}} \gets \proc{ndf-optimize}({\cal F}[{o_{tgt}}], P_{o_{tgt}}, z_q)$ 
        \State\Comment{\emph{Adapt query pose to test scene based on target object}}
        \State
        \If{$l.mode {=} \texttt{detach}$}
        \State ${\T{o_{tgt}}{e}} \gets C_{acc}[\langle{o_{tgt}, e}\rangle]$
        \State\Comment{Extract required constraints from $C_{acc}$}
        \EndIf
        \State
            \For{$z^{(t)} \in {\cal Z_{\tau}}$}
                \State ${\T{q_{tgt}}{w}^{(t)}} \gets \proc{ndf-optimize}({\cal F}[{o_{src}}], P_{o_{src}}, z^{(t)})$
                \State\Comment{\emph{Adapt motion to test scene based on source object}}
                \If{$l.mode {=} \texttt{detach}$}
                    \State ${\T{e}{w}^{(t)}} \gets {\T{q_{tgt}}{w}^{(t)}}\cdot ({\T{q_{tgt}}{o_{tgt}}})^{-1}\cdot ({\T{o_{tgt}}{e}})^{-1}$
                \Else
                    \State ${\T{e}{w}^{(t)}} \gets {\T{q_{tgt}}{w}^{(t)}}$
                \EndIf
                \State \Yield{} ${\T{e}{w}^{(t)}}$ \Comment{Yield target to controller}
            \EndFor
        \State
        \If{$l.mode {=} \texttt{detach}$}
            \State delete ${C_{acc}}$[$\langle{{o_{tgt}}, e\rangle$]\Comment{Remove constraint from $C_{acc}$}
        \Else
        \State $\T{o_{src}}{o_{tgt}} \gets \T{q_{tgt}}{o_{tgt}}\cdot (\T{q_{tgt}}{w}^{(|\tau|)})^{-1}\cdot \T{o_{src}}{w}$ 
        \State\Comment{Calculate the acquired constraint at last time step}
        \State $C_{acc}[\langle{o_{src}}, {o_{tgt}}\rangle] \gets \T{o_{src}}{o_{tgt}}$ \Comment{Append constraint to $C_{acc}$}
        \EndIf
        \State
        
        \State $\widehat{\T{o_{tgt}}{w}} \gets \T{q_{tgt}}{w}^{(|\tau|)}\cdot (\T{q_{tgt}}{o_{tgt}})^{-1}$
        \State\Comment{Calculate the expected target object pose at last time step}
        \State
        \State $\widehat{P_{o_{tgt}}} \gets {\mathit H}^{-1}(\widehat{\T{o_{tgt}}{w}}\cdot(\T{o_{tgt}}{w})^{-1}\cdot {\mathit H}(P_{o_{tgt}}))$
        \State\Comment{Compute the expected target object point cloud, ${\mathit H}(\cdot)$ means homogeneous transformation}
        \State
        \State $G[o_{tgt}] \gets \langle\widehat{P_{o_{tgt}}}, \widehat{\T{o_{tgt}}{w}}\rangle$ \Comment{Update scene graph $G$}
    \EndProcedure
\end{algorithmic}
\end{small} % footnotesize
\end{algorithm}

% Shou adapts trajectories without simulation so it's not actions
% Stacking (more general kinematics)
% Observable vs partially observable
% Offline vs online

Our first algorithm directly adapts a demonstration $d$ to the current task.
%Similar to MimicGen + NDF~\cite{mandlekar2023mimicgen}
Algorithm~\ref{alg:adaptation} displays the trajectory adaptation pseudocode.
It iterates over each \revise{$z^{(t)}$} in the feature trajectory \revise{$\cal{Z_{\tau}}$} in demonstration $d$ and computes the query transformation \revise{${\T{q_{tgt}}{w}^{(t)}}$} for the point cloud observation \revise{${P_{o_{src}}}$} in the test scene.
Depending on the skill mode, it converts \revise{${\T{q_{tgt}}{w}^{(t)}}$} into a target end-effector pose \revise{${\T{e}{w}^{(t)}}$}, which will serve as a setpoint for a downstream controller or planner.
After iterating over the feature trajectory, the scene graph is updated with the new state of the manipulated object's pose and its point cloud, which can be used for future planning and collision checking.

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=1.\linewidth]{images/skill_reasoning.pdf}
  \end{center}
  \caption{\textbf{Skill Planning and Trajectory Adaptation.} 
  On this representative mug insertion task, \Ours first selects a sequence of compatible skills by checking their NOD feature compatibility (Sec.~\ref{ssec:planning}). The trajectory is then adapted using Algo.~\ref{alg:adaptation} for the current scene. \revise{Finally, a motion planner verifies the feasibility of the end-effector's motion from the end of the preceding skill to the start of the subsequent one. It then produces transitional trajectories accordingly (Sec.~\ref{sec:motion}).}
  }
  % \vspace{-10pt}
  \label{fig:skill_reasoning}
\end{figure}


%\subsection{Task and Motion Planning}
\subsection{Skill Planning}\label{sec:plan}
\label{ssec:planning}
%Adapting an entire demonstration trajectory may be unsuitable in many cases -- for example, if the {\em plan skeleton}, or the sequence of skills changes from the reference demonstration. This motivates the capability to use segments of multiple demonstrations together. As an example, it might be possible to adapt the picking part of a pick-and-place mug demonstration to interact with a new object (a bowl, for instance), or re-use part of an existing demonstration to achieve a new goal.

% It can be limiting to be only able to reuse whole demonstrations.
% First, it is inflexible in problems where the, {\em plan skeleton}, or the sequence of skills changes.
% Second, segments of multiple demonstrations in conjunction might better address a new problem. For example, we may just transfer the picking part of the pick-and-place trajectory that work with a mug to interact with a new object, e.g., a bowl.

% https://github.com/touristCheng/robomimic-hitl/blob/c68e89334c468f3164ab04d63bc586260f7c015b/robomimic/scripts/traj_optim_full_task_%2Bmp.py#L902
\begin{algorithm}[!ht]
  \begin{small} % footnotesize
  \caption{\Ours planner}
  \label{alg:planner}
  \begin{algorithmic}[1] % The number tells where the line numbering should start
    \Declare Plan skeleton $\widehat{\pi} = [\langle l_1, o_{src_1}, o_{tgt_1} \rangle, ..., \langle l_h, o_{src_h}, o_{tgt_h} \rangle]$ % Capitalize
    \Declare Task goal specification $Z_{g}$
    \Procedure{plan-ndf-skills}{$\widehat{\pi}, Z_g, {\cal D}, {\cal F}$}
        \State $D_{\pi} = [\;]$ \Comment{List of demos per skill}
        \For{$\langle l_i, o_{src_i}, o_{tgt_i} \rangle \in \widehat{\pi}$}
            \State $D_{\pi} \gets D_{\pi} + [\{d \mid d \in {\cal D}, \langle l, o_{src}, o_{tgt}, {Z}_\textsubscript{req}, {Z}_\textsubscript{del}, {Z}_\textsubscript{add}\rangle \in d,\; \ l {=} l_i \wedge o_{src}.category {=} o_{src_i}.category \wedge o_{tgt},category {=} o_{tgt_i}.category\}]$
        \EndFor
        \State $\pi_* \gets \None$; $c_* \gets \infty$
        %\caelan{Sort instead of min?}
        \For{$\pi \in \proc{product}(D_\pi )$} \Comment{All combinations} % Cartesian product, DFS
            \State $c_\pi \gets 0$ \Comment{Feature cost}
            \State $Z_{acc} \gets \{\}$ \Comment{All accumulated constraints}
            \For{$i \in [1, ..., |\pi|]$}
                % \State $\langle o_i, f_i \rangle, \langle o_{i+1}, f_{i+1} \rangle \gets \pi[i], \pi[i+1]$
                % \State ${\cal Z}_i, {\cal Z}_{i+1} \gets \pi[i], \pi[i{+}1]$
                \State $ {Z}_\textsubscript{req}, {Z}_\textsubscript{del}, {Z}_\textsubscript{add} \gets \pi[i]$
                \For{$\langle k, z_k \rangle \in Z_\textsubscript{req}$}
                    \State $\hat{z}_{k} \gets Z_{acc}[k]$
                    \State $c_\pi \gets c_\pi + ||\hat{z}_{k} - z_k||$ % _2
                    \State\Comment{Compute feature distance among skills}
                \EndFor
                \State $Z_{acc} \gets Z_{acc} \cup Z_\textsubscript{add} \setminus Z_\textsubscript{del} $
                \State\Comment{Update acquired constraints}
            \EndFor
            \For{$\langle k, z_k \rangle \in Z_\textsubscript{g}$}
                \State $\hat{z}_{k} \gets Z_{acc}[k]$
                \State $c_\pi \gets c_\pi + ||\hat{z}_{k} - z_k||$
                \State\Comment{Compute feature distance of the goal configuration}
            \EndFor
            %\State \caelan{Goal constraints?}
            \If{$c_\pi < c_*$} \Comment{Update best plan}
                \State $\pi_* \gets \pi$; $c_* \gets c_\pi$
            \EndIf
        \EndFor
        %\caelan{Filter trajectories?}
        \State \Return $\pi_*$
    \EndProcedure
\end{algorithmic}
\end{small} % footnotesize
\end{algorithm}
% https://github.com/touristCheng/robomimic-hitl/blob/htamp_dataset_mp/robomimic/scripts/traj_optim_full_task_%2Bmp.py#L1263
Given a set of skill demonstrations, the goal of the skill planner is to select a sequence of skills that can be chained together to reach a task goal.
Algorithm~\ref{alg:planner} displays the pseudocode for the \Ours planner.
It takes in a plan skeleton $\widehat{\pi}$ that defines a sequence of skill types to consider.
% Future work
It first compiles a list of skill demonstrations in dataset ${\cal D}$ relevant to $\pi$.
Then, it iterates through all possible plans using these skills.
Each candidate $\pi$ is scored based on the compatibility of subsequent actions using NDF features, the cost $c$ is computed as
$c = \sum_{i=1}^{|\pi|}\sum_{k \in \pi[i].Z_{req}} ||z_k {-} \hat{z}_k||$
, where for specific skill demo $\pi[i]$'s required constraints (encoded as feature) $Z_{req}$, the feature $z_k$ is encoding the relative transform (constraint) of a paired object: $k=\langle{o_{src}, o_{tgt}} \rangle, z_k {\gets} F(\T{q_{tgt}}{w} \mid P_{o_{src}})$, and $\hat{z}_k$ is the corresponding feature from the acquired constraints of planned skills in previous steps. Besides evaluating skill compatibility, we also compute the cost between the goal $Z_g$ and all accumulated constraint features, and add them to the final cost.

% and $z_{i+1}$ are extracted as:
% \begin{equation*}
% z_i, z_{i + 1} \gets F(T_i \mid P), F(T_{i+1} \mid P)
% \end{equation*}

% Here $T_i$ and $T_{i+1}$ are the query pose determined at the last time step and first time step of the trajectories from skill $i$ and skill $i+1$ respectively, and $P$ is the point cloud of the target object for skill $i$ and skill $i+1$ captured during demonstration.

% \caelan{Shuo: add a standalone equation for the cost here}
After we obtain all costs for all skill combinations, the plan with the lowest plan-wide NDF feature distance is returned. For simplicity, we present this as a Cartesian product over relevant skills, but this can be done more efficiently by performing a Uniform Cost Search in plan space, where the NDF feature distance serves as a the cost function. Fig.~\ref{fig:feat_match} visualizes the feature matching process for a mug placing example.
It demonstrates that grasping the mug on its rim is compatible with placing the mug upright in a bin and grasping it on its handle is compatible with inserting it into a cabinet.

% plan-space Depth-First Search (DFS)
% Precondition?

\begin{figure}[t!]
  \begin{center}
    \includegraphics[width=1.\linewidth]{images/feat_match.png}
  \end{center}
  % \caption{\textbf{Feature Matching.} The feature matching distance for different skill combinations when placing a mug. In this example, for characterizing the relationship between the mug and the end-effector, we use the NOD feature extracted from the mug point cloud and the end-effector pose in the mug frame, for representing the relationship between mug and cabinet, we use the NOD feature extracted from the mug point cloud and the cabinet pose.}
  \caption{\textbf{Feature Matching.} \revise{We visualize the NOD feature distance of different skill combinations from the pick and place mug example, where darker color map represents lower matching cost.} The NOD feature extracted from the mug point cloud and the end-effector pose is used to characterize the relationship between the mug and the end-effector, and the NOD feature extracted from the mug point cloud and the container (e.g., cabinet) pose is used to represent the relationship between the mug and the container. Grasping the mug on its rim is compatible with placing the mug upright in a bin and grasping the mug on its handle is compatible with inserting it into a cabinet. This allows \Ours to adapt different demonstration pieces to accomplish different goals.}
  \label{fig:feat_match}
  \vspace{-10pt}
\end{figure}


%\subsection{Motion Planning}
%\subsection{Motion Refinement}
\subsection{Transit \& Transfer Motion}
\label{sec:motion}

Adapting demonstrated skills is particularly effective at generating behavior that involves contact.
However, demonstrations typically contain long segments without contact (outside of holding an object). Because these components do not modify the world, it is often not productive to replicate them.
Thus, we temporally trim skill demonstrations to focus on the data points that involve contact. In our implementation, we simply select the 50 steps before contact.
% \caelan{Shuo: give specific criteria}

After trimming, and in often before trimming, two adjacent skills might be far away in task space.
While linear interpolation is an option, this is not generally safe because the straight-line path may cause the robot to unexpectedly collide.
To address this, we use motion planning to optimize for safe and efficient motion that reaches the start of next the skill.
Motion planning generally requires some characterization of the collision volume of the obstacles to avoid.
Because we do not assume access to object models, we use the segmented point clouds ${\cal P}$ as the collision representation, where each point in the cloud is a sphere with radius $r > 0$.

\begin{algorithm}[!ht]
  \begin{small} % footnotesize
  \caption{\Ours policy}
  \label{alg:policy}
  \begin{algorithmic}[1] % The number tells where the line numbering should start
  \Declare task goal constraints $C_g$
  \Declare Plan skeleton $\widehat{\pi} = [\langle l_1, o_{src_1}, o_{tgt_1} \rangle, ..., \langle l_h, o_{src_h}, o_{tgt_h} \rangle]$ % Capitalize
    \Procedure{\Ours-policy}{${\cal P}, C_g, \widehat{\pi}; {\cal D}, {\cal F}$}
        \State $G \gets \proc{init-scene-graph}({\cal P}, {\cal D}, {\cal F})$
        \State $Z_g \gets \proc{compute-goal-feature}({\cal P}, C_g, {\cal F})$
        \State $\pi \gets \proc{plan-ndf-skills}(\widehat{\pi}, Z_g; {\cal D}, {\cal F})$
        \If{$\pi = \None$}
            \State \Return \False \Comment{Skill planning failed}
        \EndIf
        % \State $q \gets \proc{observe-conf}()$
        % \State $\R{S}{e}{w} \gets \proc{forward-kin}(q)$
        \For{$d \in \pi$}
        \State $o_{src}, o_{tgt} \gets d$
        \State $a \gets \True$ \Comment{Starting of the skill}
        \For{$\R{T}{e}{w} \in \proc{adapt-traj}(o_{src}, o_{tgt}, d; {\cal F}$)}
            \If{$a = \True$}
                \State $a \gets \False$
                \State $q \gets \proc{observe-conf}()$
                \State $\tau \gets \proc{plan-motion}({\cal P}, q, \R{T}{e}{w})$
                \If{$\tau = \None$}
                    \State \Return \False \Comment{Motion planning failed}
                \EndIf
                \State $\proc{execute-traj}(\tau)$
            \EndIf
            \State $q \gets \proc{observe-conf}()$
            \State $\proc{execute-osc}(q, \R{T}{e}{w})$ \Comment{Operational Space}
            
        \EndFor
        \EndFor
        %\State \proc{adapt-trajectory}($S_0, \pi$)
        \State \Return \True \Comment{Policy succeeded}
    \EndProcedure
\end{algorithmic}
\end{small} % footnotesize
\end{algorithm}
%\caelan{What exactly are the goal constraints in our domains?}
%\caelan{Sum of task score and comp score}
% Observation where the observation could just be the state
% Label $l = \langle x, f, f' \rangle$
% Vector notation for a plan
% Different labels per pair for frames
% Online vs offline
% Learned action constraints
% Plan-space planner

Algorithm~\ref{alg:policy} displays the pseudocode for the full \Ours policy with motion planning.
It is shown with online motion planning and execution, but full plans can also be computed offline.
The policy first computes a skill plan $\pi$ and then adapts each labeled trajectory in sequence.
Between adapted trajectories, it uses \proc{plan-motion} to plan a trajectory from the current robot configuration $q$ to a configuration that reaches the first end-effector pose $\R{T}{e}{w}$.
Specifically, it samples goal configurations $q'$ using inverse kinematics and then invokes a sampling-based motion planner between $q$ and $q'$.
% Holding
Once the end-effector arrives at $\R{T}{e}{w}$, for each pose yielded by the skill, the policy uses an Operational Space Controller (OSC)~\cite{khatib1987unified} to track the target poses. 

A detailed example of how the system works for placing the mug into the cabinet is presented in Fig.~\ref{fig:skill_reasoning}. The skill planning process first identifies the reference trajectories for the pick and place skills by matching constraint features (see Fig.~\ref{fig:feat_match} for an example).
These trajectories are adapted to the test scene using NDFs.
Then, a motion planner generates transitory motion between these trajectories. 
% Once the motion transition among every connections between the consecutive skills are determined, we transfer the trajectories to the test scene through trajectory adaptation. 
Altogether, the planning time is typically 1-2 minutes, where the NDF optimization is most of the runtime.
These algorithms can be run online while the robot is executing to minimize the overall task time.


==> text/Problem.tex <==
\newpage
%\section{Problem Formulation \todo{remove later}}
\section{Brainstorm \todo{remove later}}

\caelan{Adding new content to section "Background" instead of here. The figures in this section could evolve into a nice example though.}
%\caelan{This closely follows the notation used in the NDF papers. We don't necessarily need to do that, especially since we aren't inovating within NDFs.}

\caelan{TODO(Shuo): equation that evaluates the Skill Reasoning distance}

\subsection{NDF Representation}
\noindent\textbf{Invariant to Category-level Shape Changes (Shape Generalization)} Neural Descriptor Fields (NDF) models take in an object shape that is represented as a point cloud $P \in \mathbb{R}^{N\times3}$ and a set of query positions $\{R \cdot x_i+t| \forall x_i \in X\}$ (where $[R\;|\;t] = T\in\mathbb{R}^{4\times4}$ is a transform, and $X \in \mathbb{R}^{M\times3}$ is the original query points), and output the features corresponding to the queries:

\begin{equation}
\posedescriptor = \posendf(T | P) = \bigoplus_{x_i \in X} \pointndf( R\cdot x_i+t| P)
\label{eq:pose_enc}
\end{equation}


Since the NDF encoder is trained with diverse object shapes, therefore it will assign similar features to the queries even if we change the object shape to be a new one (denoted as $P^{'}$), as long as the new queries are at the positions (the new transform is denoted as $T^{'}=[R^{'}|t^{'}]$) that are geometric equivalent to the original queries w.r.t. the object shape (See Fig.~\ref{fig:ndf_pose}):

\begin{figure}
  \begin{center}
    \includegraphics[width=0.8\linewidth]{images/NDF_pose.pdf}
    \vspace{-5pt}
  \end{center}
  \caption{Illustration of using NDF for transferring pose to a new object $P^{'}$ based on reference object $P$ and pose $[R|t]$.}
  \label{fig:ndf_pose}
  \vspace{-10pt}
\end{figure}

\begin{equation}
\posedescriptor = \bigoplus_{x_i \in X} \pointndf( R\cdot x_i+t|P) = \bigoplus_{x_i \in X} \pointndf( R^{'}\cdot x_i+t^{'}|P^{'})
\label{eq:pose_enc}
\end{equation}

Given a reference pose $T$ and a reference object $P$, we can first obtain the corresponding feature $\posedescriptor$. To obtain the new pose $T^{'}$ that maps points from the base frame to the geometric equivalent positions in the new shape's frame, we can randomly initialize the new pose and back-propagate the gradient to it: 

\begin{equation}
T^{'} = \underset{T^{'}}{\text{argmin}} ||\posedescriptor, \posendf(T^{'}|P^{'})||.
\label{eq:pose_enc}
\end{equation}

Given any point in the base frame, the obtained new pose $T^{'}$ will transform the point to the position that is geometric equivalent (w.r.t. the new object shape) to the one mapped by the reference pose $T$ (w.r.t. the reference object shape).

\textbf{Invariant to Joint Transformation (Pose Generalization):} Since the NDF feature is only related to the queries in the object's local frame, therefore a joint transform $T^{c}\in \mathbb{R}^{4\times4}$ applied to both the shape and the query pose would affect the extracted feature, which allows us to generalize the extracted pose $T^{c}T^{'}$ with arbitrary configuration $T^{c}$ of the new shape:

\begin{equation}
\posedescriptor = \posendf(T | P) = \posendf(T^{c}T^{'} | T^{c}P^{'}) 
\label{eq:pose_enc}
\end{equation}

\subsection{NDF for Long-horizon Manipulation}

\caelan{We need to be careful that this doesn't come across as TAMP with category-level pose estimation instead of conventional pose estimation. At the very least wrt constraints, we're estimating frames that define action constraints (e.g. grasp \& insertion poses).}

\textbf{Object Pose Extraction:}
To obtain the object pose in the base frame, we can specify the reference queries to be at the center of the reference object (treating the reference object as the same orientation as its canonical frame), record the reference feature, and use it to optimize the pose for the new object shape. 

\caelan{Good, after describing the generic NDF framework. We'll want to clearly describe the interaction types we consider in our experiments. }

\textbf{Object Interaction Modeling:}
For modeling the interaction between two objects (e.g., gripper-peg, or peg-hole), we can specify the query point to be at the contact region of the first object, and extract the NDF feature of the queries w.r.t. the second object. Take peg-hole as an example (See Fig.~\ref{fig:ndf_interact}), we need to track the motion of the contact part (green queries) of the peg instead of the center (red queries), as different pegs may have different lengths (thus different transforms between peg center to peg contact region). 

\begin{figure}
  \begin{center}
    \includegraphics[width=0.9\linewidth]{images/NDF_interaction.pdf}
    \vspace{-5pt}
  \end{center}
  \caption{Illustration of generating motion trajectory for test scenario based on the reference demonstration.}
  \label{fig:ndf_interact_}
  \vspace{-10pt}
\end{figure}

A general way to model object-object interaction is to define two queries for each reference object, one at the object center, and one at the contact part. Let $P^{ref\_tool}$ and $P^{test\_tool}$ be the reference tool object and test tool object, $P^{ref\_recep}$ and $P^{test\_recep}$ be the reference receptacle and test receptacle, and let $\posendf_{tool}(\cdot|\cdot)$ and $\posendf_{recep}(\cdot|\cdot)$ be the NDF model for tool and receptacle. 

\caelan{We haven't gotten to true relational interactions where an NDF consumes both point clouds at the same time, right?}

We first record the corresponding feature $\posedescriptor_{center}$ and $\posedescriptor_{contact}$ for center and contact part of the reference tool object, we can then extract the pose for center $T_{test\_tool\_center}$ and pose for contact part $T_{test\_tool\_contact}$ of the test tool object with $\posendf_{tool}(\cdot|\cdot)$:

\begin{equation*}
T_{test\_tool\_center} = \underset{T}{\text{argmin}} ||\posedescriptor_{center}, \posendf_{tool}(T|P^{test\_tool})||
\label{eq:pose_enc}
\end{equation*}

\begin{equation*}
T_{test\_tool\_contact} = \underset{T}{\text{argmin}} ||\posedescriptor_{contact}, \posendf_{tool}(T|P^{test\_tool})||
\label{eq:pose_enc}
\end{equation*}

The transform from the tool contact region to the tool frame can be computed as $T_{contact\_to\_test\_tool} = T_{test\_tool\_center}^{-1}\cdot T_{test\_tool\_contact}$.
Similarly, we can obtain the pose of the gripper frame $T_{gripper\_center}$, and the pose of the tool $T_{test\_tool\_center}$ at the time when the robot close the gripper, the grasp pose can then be represented as $T_{test\_tool\_to\_gripper} = T^{-1}_{gripper\_center}\cdot T_{test\_tool\_center}$. The transform from the contact frame to the gripper frame can finally be computed as: $T_{contact\_to\_gripper} = T_{test\_tool\_to\_gripper}\cdot T_{contact\_to\_test\_tool}$. \textcolor{red}{Once we are able to track the motion of the contact part of the tool object}, we can use this transform to derive the motion of the gripper for controlling robot.

Given the reference motion $\tau$ from the demonstration, we first extract the corresponding feature $\posedescriptor_i$ for each pose $T_{i}=[R|t]_{i} \in \tau$ with the $\posendf_{recep}(\cdot|\cdot)$:

\begin{equation}
\posedescriptor_i = \posendf_{recep}(T_i | P^{ref\_recep})
\end{equation}

We can then generate the motion $\tau^{'}$ for the test scenario by optimizing each corresponding pose $T^{'}$ of the contact part of the test tool:

\begin{equation}
T_{i}^{'} = \underset{T}{\text{argmin}} ||\posedescriptor_{i}, \posendf_{recep}(T|P^{test\_recep})||
\end{equation}

\caelan{Discuss optimizing sequentially via warm starts}

An additional advantage of this geometric-equivalent feature is that it allows us to generalize the grasping strategies to new grippers, as we can first align the contact region of the finger and then derive the gripper pose.

\noindent\textbf{Automatic Identification of Contact and Centroid Parts for Reference Objects} During demo collection, we can compute the center of each reference object point cloud, and we can treat them as at the identical orientation, therefore, we do not need to manually place the queries for extracting the object frame. For identifying the contact part, one way is to compute the motion direction of the tool object, the contact part should be at the intersection of the tool object surface and motion direction (See Fig.~\ref{fig:contact}), as when the contact part hit the receptacle, the motion stops. Another way is directly detect the closest point between two objects. In this way, we can relax the assumption that the user needs to specify the queries, we only need RGB-D perception and instance-level object segmentation.
\caelan{Could move to the main text}

\begin{figure}
  \begin{center}
    \includegraphics[width=0.5\linewidth]{images/contact.pdf}
    \vspace{-5pt}
  \end{center}
  \caption{Illustration of contact region identification.}
  \label{fig:contact}
  \vspace{-10pt}
\end{figure}

\noindent\textbf{NDF-augmented Operators}

TODO

\noindent\textbf{Search Forward and Backtracking} Since we are able to extract the absolute pose for any object and its parts, and estimate the ending pose of given motion trajectory, we can generate (through rigid transformation) the future configuration of the resulting scene after successful execution. We will use the generated scene that represented as point cloud for collision checking (maybe implemented as neural network) and trajectory ranking. 

\subsection{Implementation and Experiment Design}
\noindent\textbf{Major To-do}
\begin{itemize}
    \item Verify NDF for trajectory generation; [x]
    \item Verify NDF for long-term manipulation (including obj-obj interaction, simple task); [ ]
    \item Reproduce HITL-TAMP system, integrate NDF; [ ]
    \item Build full task environment (mug place, tool usage), train NDF models on new shapes; [ ]
\end{itemize}

\noindent\textbf{Experiments}
\begin{itemize}
    \item Show generalization to different configurations and shapes;
    \item Show generalization to different grippers and even different robots;
\end{itemize}

\subsection{Conclusion}
NDF descriptor field allows us to find geometric equivalent positions across different objects, it is more like implicit kinematics chains where we can use it to propagate transforms between objects and parts.

==> text/Rebuttal.tex <==
\clearpage
% \newpage\hbox{}\thispagestyle{empty}
\newpage

\section{Rebuttal}

We thank the reviewers for their time and constructive suggestions. We are grateful for the positive recognition of the reviewers on our work’s novelty (\textcolor{red}{rDtH-AC}, \textcolor{cyan}{usKg-R1}, \textcolor{orange}{SuUa-R3}), impressive data efficiency (\textcolor{red}{rDtH-AC}, \textcolor{orange}{SuUa-R3}), and the capability of handling diverse generalization challenges in long-horizon tasks within a unified framework (\textcolor{red}{rDtH-AC}, \textcolor{cyan}{usKg-R1}, \textcolor{violet}{SevE-R2}) that relaxes the constraints of engineering the skills and perception for classical TAMP system (\textcolor{orange}{SuUa-R3}). We address the concerns in detail below and in the revision. 

\textbf{Clarity of Presentation} (\textcolor{red}{AC}, \textcolor{cyan}{R1}, \textcolor{violet}{R2}, \textcolor{orange}{R3}): 
%We recognize that the presentation of our method may have lacked clarity and intuitive explanation, and we extend our gratitude to all the reviewers for the helpful feedback. In response, 
We have substantially revised the writing of the Problem Formulation and the main Method section to be much easier to follow, with much fewer notations. We have also incorporated additional technical details in the revised version. % \ajay{first mention that the presentation was revised to be much easier to follow, then mention that some technical details were also added}. % Specifically:

% \danfei{No longer true I think. We can get rid of the su}
% \begin{itemize}
%     \item In Section IIIA, we define $\pointndf$ as a learned model that maps a single query coordinate to a feature vector, and $\posendf$ as an operation that maps a query pose to an extended feature descriptor by concatenating all the features of a set of query coordinates parameterized by the query pose;
%     \item We define $P_o$ as the object point cloud from the perception;
%     \item We have reworded Sec.~\ref{sec:problem} to make it more clear;
%     \item We have simplified notations in Fig.~\ref{fig:ndf_interact}, and included additional explanations for Fig.~\ref{fig:ndf_interact}, Fig.~\ref{fig:skill_reasoning}, and Fig.~\ref{fig:feat_match};
% \end{itemize}

\textbf{New Real-world Long-horizon Contact-rich Tasks} (\textcolor{red}{AC}, \textcolor{cyan}{R1}, \textcolor{violet}{R2}, \textcolor{orange}{R3}): Given that our system requires only a small number of demonstrations across a select few target objects, it lends itself readily to deployment in real world scenarios, particularly those involving long-horizon tasks. To validate the system's capability to address long-horizon contact-rich manipulation, we experimented on two new real-world tasks:
\begin{itemize}
    \item \textbf{Make Coffee}: This task consists of 6 stages: 1) pick the coffee pod, 2) insert the pod, 3) pick the mug, 4) place the mug in the coffee machine, 5) close the coffee machine's lid, and 6) press the coffee machine's button to turn it on. 
    % It was considered as long-horizon tasks as each stage may already need hundred of time steps \ajay{I would remove this part -- number of timesteps is an arbitrary measure} for a learned policy to complete~\cite{zhu2022viola, mandlekar2023mimicgen}, 
    The insert pod skill requires the robot to carefully align the pod with the holder of the coffee machine, demonstrating contact-rich manipulation. 
    \item \textbf{Sort Tableware}: This task also consists of 6 stages: pick and insert the plate into the slot and then stack two bowls on the rack.
\end{itemize}

On the \textbf{Make Coffee} task, \Ours achieves a 60\% success rate over 10 trials, where the pod and mug randomly placed on a center region of the table.
On the \textbf{Sort Tableware} task, \Ours achieves a 90\% success rate over 10 trials . We provide more details on the testing process and performance analysis, in Sec.~\ref{sec:real_exp} and Sec.~\ref{sec:real_res}.

\textbf{Analysis of Robustness to Perception Noise} (\textcolor{red}{AC}, \textcolor{cyan}{R1}, \textcolor{violet}{R2}) To quantitatively evaluate robustness to perception noise, in simulation, we inject different levels of random noise into the observed point cloud and run \Ours.
See Sec.~\ref{sec:perception_noise} for a description of the experiment. In addition, we visualize the captured objects in the real-world along with the predicted trajectories in Fig.~\ref{fig:real_res}. Despite the noisy perception in the real world, our system is able to solve these tasks with good success rates. %\ajay{I suggest highlighting any additional results on robustness to perception noise in simulation first if possible. Also highlight that real-world perception is noisy, and despite this, we can solve challenging tasks (and highlight the recent new results as well)}.

\textbf{Demonstration Data Details} (\textcolor{red}{AC}, \textcolor{orange}{R3}) We visualize the reference skill trajectories for the real-world tasks in Fig.~\ref{fig:real_demos}. All of the reference demos are collected by a human through kinesthetic teaching. More details on demo processing and skill representations are presented in Sec.~\ref{sec:demo_collect}
% we also tested the system with programmed motions, the analysis can be found in Sec.\shuo{TBD}. \ajay{Perhaps summarize the additional details here (e.g. how data was collected in sim and real, with teleoperation, kinesthetic teaching, etc))}

\textbf{Analysis of Sensitivity to Imperfect Demos} (\textcolor{orange}{R3}) 
% To analyze the sensitivity of our system to demo quality, we report its performance on real-world task with various reference demos in the revised version Sec.~\ref{sec:demo_quality}. \ajay{Make it more clear how this addresses the question -- e.g. what is imperfect about the demos in this analysis?}
To analyze how demo quality affects the performance of our system, we use the ``Can" task from Robomimic benchmark~\cite{robomimic2021} to test our system, which paired with hybrid human demos. According to Robomimic, the demos are categorized into three groups with quality ``better", ``okay", and ``worse". We randomly sampled 4 demos from each group, and we run 10 trials for each source demo with randomly initialized object placements, the results are presented in Fig.~\ref{fig:demo_qual}. The results show that our system’s performance correlates with the quality of the reference demonstrations, similar to other learning from demonstration methods. We found that our system is robust to sub-optimal trajectories, e.g., the robot gripper takes indirect path to approach the object. We also notice that some of the failure cases come from the slippery of the object, probably due the sub-optimal grasp pose, incorporating failure detection and re-planning capability would be able to mitigate this issue.

\textbf{Comparison with Learned Control Policies} (\textcolor{violet}{R2}): We compare our system with other end-to-end policy learning methods on the LIBERO benchmark, where all baselines are trained with the official benchmark teleoperation data.
%released by the benchmark that contains exactly the same object shapes used during testing. 
We report their performances directly from the leader board. Note that all Behavior Cloning methods require large volumes of data. In constrast, \Ours only requires a handful of examples. The neural object descriptors used in our system are trained purely using object shape data in simulation, without the need of any robot trajectories. %\ajay{This part is unclear - do you mean the NDFs? This sentence feels a little out of place. I would first highlight the positives -- e.g. BC typically requires large volumes of data, while our method works using a handful of examples. Then you can mention that the NDF models used by our method purely use object models for training, without any robot trajectories.}. 
During deployment, only a handful of demonstrations are needed, without requiring any further training or fine-tuning.

Since end-to-end policy learning approaches (e.g., Behavior Cloning) typically need a substantial volume of teleoperation data for training, evaluating such methods on tasks lacking such training data poses a non-trivial challenge. (e.g., all proposed tasks in Tab. 2, and all real-world tasks). 

\textbf{Collision Checking during Motion Planning} (\textcolor{violet}{R2}) In our framework, motion planning is used to generate free space motions between skills. Because the starting frame of each skill is typically distant from objects, this mitigates the need for precise scene geometry representations during collision checking, potentially offering another advantage of our method.

\textbf{On the ``Contact-rich'' Terminology} (\textcolor{cyan}{R1}) 
%We thank the reviewer for bringing up this point. 
While most of the evaluation tasks do involved multiple object-object contacts, we agree that ``contact-rich'' may not be the appropriate term.
%can be perceived as overclaiming. 
Thus, we modified our terminology to use ``fine-grained'' manipulation to better reflect the nature of the evaluation tasks.
%and the requirement of adapting human-demonstrated trajectories.
